Testing Positive Semi-Definiteness via Random Submatrices

We study the problem of testing whether a matrix $\mathbf{A} \in \mathbb{R}^{n \times n}$ with bounded entries ($\|\mathbf{A}\|_\infty \leq 1$) is positive semi-definite (PSD), or $\epsilon$-far in Euclidean distance from the PSD cone, meaning that $\min_{\mathbf{B} \succeq 0} \|\mathbf{A} - \mathbf{B}\|_F^2 > \epsilon n^2$, where $\mathbf{B} \succeq 0$ denotes that $\mathbf{B}$ is PSD. Our main algorithmic contribution is a non-adaptive tester which distinguishes between these cases using only $\tilde{O}(1/\epsilon^4)$ queries to the entries of $\mathbf{A}$. If instead of the Euclidean norm we considered the distance in spectral norm, we obtain the "$\ell_\infty$-gap problem", where $\mathbf{A}$ is either PSD or satisfies $\min_{\mathbf{B}\succeq 0} \|\mathbf{A}- \mathbf{B}\|_2 > \epsilon n$. For this related problem, we give a $\tilde{O}(1/\epsilon^2)$ query tester, which we show is optimal up to $\log(1/\epsilon)$ factors. Our testers randomly sample a collection of principal submatrices and check whether these submatrices are PSD. Consequentially, our algorithms achieve one-sided error: whenever they output that $\mathbf{A}$ is not PSD, they return a certificate that $\mathbf{A}$ has negative eigenvalues. We complement our upper bound for PSD testing with Euclidean norm distance by giving a $\tilde{\Omega}(1/\epsilon^2)$ lower bound for any non-adaptive algorithm. Our lower bound construction is general, and can be used to derive lower bounds for a number of spectral testing problems. As an example of the applicability of our construction, we obtain a new $\tilde{\Omega}(1/\epsilon^4)$ sampling lower bound for testing the Schatten-$1$ norm with a $\epsilon n^{1.5}$ gap, extending a result of Balcan, Li, Woodruff, and Zhang [SODA'19]. In addition, it yields new sampling lower bounds for estimating the Ky-Fan Norm, and the cost of the best rank-$k$ approximation.

==> Abstract.tex <==
%We study the problem of testing whether a matrix $A \in \R^{n \times n}$ with bounded entries ($\|A\|_\infty \leq 1$)  is positive semi-definite (PSD), or $\eps$-far in $\ell_2^2$-distance from the PSD cone, i.e.  $\min_{ B \succeq 0} \| A - B\|_F^2  = \sum_{i : \lambda_i(A) < 0} \lambda_i^2(A) > \eps n^2$.
   % Our main algorithmic contribution is a non-adaptive tester which distinguishes between these cases using only $\tilde{O}(1/\eps^4)$ queries to the entries of $A$. For the related ``$\ell_\infty$-gap problem'', where $A$ is either PSD or has an eigenvalue satisfying $\lambda_i(A) < - \eps n$, our algorithm only requires $\tilde{O}(1/\eps^2)$ queries, which is optimal up to $\log(1/\eps)$ factors.     Our testers randomly sample a collection of principle sub-matrices and check whether these sub-matrices are PSD. Consequentially, our algorithms achieve \textit{one-sided error}: whenever they output that $A$ is not PSD, they return a certificate that $A$ has negative eigenvalues.
    
 %  We complement our upper bound for PSD testing with $\ell_2^2$-gap by giving a $\tilde{\Omega}(1/\eps^2)$ lower bound for any non-adaptive algorithm.  Our lower bound construction is general, and can be used to derive lower bounds for a number of spectral testing problems. As an example of the applicability of our construction, we obtain a new $\tilde{\Omega}(1/\eps^4)$ sampling lower bound for testing the Schatten-$1$ norm with a $\eps n^{1.5}$ gap,   extending a result of Balcan, Li, Woodruff, and Zhang [SODA'19] In addition, our hard instance results in new sampling lower bounds for estimating the Ky-Fan Norm, and the cost of rank-$k$ approximations, i.e.  $\|A - A_k\|_F^2 = \sum_{i > k} \sigma_i^2(A)$. 
 
    We study the problem of testing whether a matrix $\mathbf{A} \in \mathbb{R}^{n \times n}$ with bounded entries ($\|\mathbf{A}\|_\infty \leq 1$)  is positive semi-definite (PSD), 
    or $\epsilon$-far in Euclidean distance from the PSD cone, meaning that $\min_{\mathbf{\BB} \succeq 0} \|\mathbf{A} - \mathbf{B}\|_F^2  > \epsilon n^2$, where $\mathbf{B} \succeq 0$ denotes that $\mathbf{B}$ is PSD.
    Our main algorithmic contribution is a non-adaptive tester which distinguishes between these cases using only $\tilde{O}(1/\epsilon^4)$ queries to the entries of $\mathbf{A}$. If instead of the Euclidean norm we considered the distance in spectral norm, we obtain the ``$\ell_\infty$-gap problem'', where $\mathbf{A}$ is either PSD or satisfies $\min_{\mathbf{B}\succeq 0} \|\mathbf{A}- \mathbf{B}\|_2  > \epsilon n$. For this related problem, we give a $\tilde{O}(1/\epsilon^2)$ query tester, which we show is optimal up to $\log(1/\epsilon)$ factors. 
  Both our testers randomly sample a collection of principal sub-matrices and check whether these sub-matrices are PSD. Consequentially,  our algorithms achieve \textit{one-sided error}: whenever they output that $\mathbf{A}$ is not PSD, they return a certificate that $\mathbf{A}$ has negative eigenvalues.
    
   We complement our upper bound for PSD testing with Euclidean norm distance by giving a $\tilde{\Omega}(1/\epsilon^2)$ lower bound for any non-adaptive algorithm. 
  Our lower bound construction is general, and can be used to derive lower bounds for a number of spectral testing problems. As an example of the applicability of our construction, we obtain a new $\tilde{\Omega}(1/\epsilom^4)$ sampling lower bound for testing the Schatten-$1$ norm with a $\epsilon n^{1.5}$ gap, 
   extending a result of Balcan, Li, Woodruff, and Zhang \cite{BalcanTesting}. In addition, our hard instance results in new sampling lower bounds for estimating the Ky-Fan Norm, and the cost of rank-$k$ approximations, i.e.  $\|\mathbf{A} - \mathbf{A}_k\|_F^2 = \sum_{i > k} \sigma_i^2(\mathbf{A})$.


==> L2GapOld.tex <==



\section{A One-Sided Tester for Positive Semi-Definiteness Matrices with $\ell_2$ Gap}
Let $\AA \in \R^{n \times n}$ be symmetric with eigenvalues $\lambda_{\max} = \lambda_1 \geq \lambda_2 \geq \dots \geq \lambda_n = \lambda_{\min}.$ Let $t \in \{0,1,\dots,n\}$ be such that $\lambda_i < 0$ for all $i \geq t$. In this section, we consider the $L_2$ gap. Namely, we are promised that $\|\AA\|_\infty \leq 1$, and that one of the two following cases hold:

\begin{enumerate}
    \item $\AA$ is PSD.
    \item $\AA$ is $\eps$-far from PSD, meaning that $\frac{\sum_{i\geq t} \lambda_i^2}{n^2} = \eps$.
\end{enumerate}
Our goal is to distinguish between the two cases. Our algorithm will query a principle submatrix $\AA_{S  \times S}$ and return PSD if $\AA_{S  \times S}$ is  PSD, otherwise it will return not PSD. Since all principle submatrices of PSD matrices are PSD, we only need show that if $\AA$ is $\eps$-far from PSD, then we can find a non-PSD principle submatrix with small size $|S|^2$. Thus, in the following, we can focus on the case where $\AA$ is $\eps$-far from PSD. 

For notation, let $\alpha \in (\eps,1]$ be such that $\|\AA\|_F^2 = \alpha n^2$.  Note that $\alpha \geq \eps$ because we have $\sum_{i} \lambda_i^2 \geq  \eps n^2$ by assumption. 
We can write $\AA = \sum_{i=1}^n \lambda_i v_i v_i^T$ where $v_1,\dots,v_n \in \R^n$ are the orthonormal eigenvectors for $\AA$, and then write $\AA$ via a cannonical decomposition $\AA = \AA^+ + \AA^-$ where $\AA^+ = \sum_{i< t} \lambda_i v_i v_i^T$ and $\AA^- = \sum_{i\geq t} \lambda_i v_i v_i^T$. Note by assumption, $\|\AA^-\|_F^2 = \eps n^2$, and by Pythagorean theorem $\|\AA\|_F^2 = \|\AA^+\|_F^2 + \|\AA^-\|_F^2$. 

\begin{lemma}\label{lem:samplefrob}
    Let $S \subset [n]$ be a random subset of expected size $k = O(\delta^{-1}(\frac{  \sqrt{c_1} }{\eps} + \frac{c_0}{\eps^2}))$. Fix a symmetric matrix $\AA \in \R^{n \times n}$ with $\sum_i \|\AA_{i,*}\|_2^4 \leq c_0 n^3$  and $\|\AA\|_4^4 \leq c_1 n^2$ for some values $c_0,c_1$. Then with probability $1-\delta$, we have $\frac{n^2}{k^2}\|\AA_{S \times S}\|_F^2 =  \|\AA\|_F^2 \pm \eps n^2 $. 
\end{lemma}
\begin{proof}
Let $\delta_i$ indicate that we choose $i \in [n]$ to add to $S$. Then $\ex{\delta_i} = \frac{k}{n}$, and 
\[\ex{\sum_{i \neq j} \delta_i \delta_j \AA_{i,j}^2 } = \frac{k^2}{n^2} \sum_{i \neq j} \AA_{i,j}^2 \] 

Moreover,
\begin{equation}
    \begin{split}
        \textbf{Var}\left(    \sum_{i \neq j} \delta_i \delta_j \AA_{i,j}^2 \right) &\leq \frac{k^4}{n^4} \sum_{4 = |\{i,j,s,r\}|} \AA_{i,j}^2 \AA_{s,r}^2 +  \frac{k^3}{n^3} \sum_{3 = |\{i,j,s,r\}|} \AA_{i,j}^2 \AA_{s,r}^2 +  \frac{k^2}{n^2} \sum_{2 = |\{i,j,s,r\}|} \AA_{i,j}^4\\ 
         - &\frac{k^4}{n^4} (\sum_{i \neq j} \AA_{i,j}^2)^2 \\  
         & \leq \frac{k^3}{n^3} \sum_{3 = |\{i,j,s,r\}|} \AA_{i,j}^2 \AA_{s,r}^2 +  \frac{k^2}{n^2} \|\AA\|_4^4\\ 
             & \leq \frac{k^3}{n^3}\sum_{i} 6\mathcal{R}_i^2  +  \frac{k^2}{n^2} \|\AA\|_4^4\\ 
    \end{split}
\end{equation} 
where $\mathcal{R}_i = \sum_{j} \AA_{i,j}^2 = \mathcal{C}_i = \sum_j \AA_{j,i}^2$. Thus  $\frac{k^3}{n^3}\sum_{i} 6\mathcal{R}_i^2 \leq \frac{k^3}{n^3} 6 c_0^2 n^3 = 6 c_0 k^3$.  Moreover, note that $\|\AA\|_4^4 \leq n^2 c_1$. Thus the variance is bounded by $6 c_0 k^3 + k^2 c_1$. So 
\[  \pr{ \sum_{i \neq j} \delta_i \delta_j \AA_{i,j}^2 -  \frac{k^2}{n^2} \sum_{i \neq j} \AA_{i,j}^2| > \eps k^2 } \leq \frac{6 c_0 k^3 + k^2 c_1}{\eps^2 k^4} \]


Finally, note that the diagonal can effect $\|\AA_{S \times S}\|_F^2$ by at most $c_0  k < \eps k^2$, thus we can add this additional $\eps k^2$ term into the overall error. 

 
\end{proof}

\begin{lemma}\label{lem:eigpreserve}
    Fix any $\eps >0$ and $x \in \R^n$ such that $|x^T \AA x| > \eps_0 n$ for some $\eps_0 > \eps$. Let $S \subset [n]$ be a random subset of size $|S| =O(\delta^{-1}/\eps^2)$. Let $Z = \AA_{S \times S}$. Then 
    \[ \bpr{    \left| \frac{n}{k}\|x_S\|_2^{-2} x^T_SZx_S - x^T \AA x \right| > \eps n    } <  \delta \]
\end{lemma}
\begin{proof}
  First note that $\|x_S\|_2^2 = (1 \pm \eps)\frac{k}{n}$. The remaining results follow from the first section.
  

\end{proof}


\subsection{A $\poly(\log(n)/\eps)$-query algorithm}

In the following, let $\| \AA \|$ denote the standard operator norm of a matrix $\AA$, and let $\|\AA \|_p = \left( \sum_{i,j} |\AA_{i,j}|^p \right)^{1/p}$ denote the $p$-norm of the vectoization of $\AA$. Let $\|\AA\|_{1 \to 2}$ denote the maximum $\ell_2$ norm of a column of $\AA$. Finally, for a random variable $X$ and $p \geq 1$, let $\mathbb{E}_p X = \left(\ex{ X^p}\right)^{1/p}$. 


\begin{theorem}[Theorem 1 \cite{tropp2008norms}]\label{thm:tropp}
Let $\AA \in \R^{n \times n}$ be Hermitian, decomposed into diagonal and off-diagonal parts $\AA = \DD + \HH $. Fix $p \geq 2$ and set $q = \max\{ p , 2\log(n)\}$. Then
\[  \mathbb{E}_p \|\RR \AA \RR \| \leq C \left[q \mathbb{E}_p \|\RR \HH \RR \|_\infty + \sqrt{\delta q} \mathbb{E}_p \|\HH \RR \|_{1 \to 2} + \delta \|\HH \|  \right]    + \mathbb{E}_p \|\RR \DD \RR \|       \]   
Where $\RR $ is a diagonal matrix with diagonal entry $\RR _{i,i} = \delta_i$ where $\delta_i$ is Bernoulli with mean $\delta$.
\end{theorem}

Recall that $\lambda_1 \geq \lambda_2 \geq \dots \geq \lambda_n$ are the eigenvalues of $\AA$, and $v_i$ is the $i$-th eigenvector of $\AA$, so that $\AA v_i = \lambda_i v_i$. Note that we can assume that $\lambda_i \geq - \eps^2 n / 1000$ for all $i$, otherwise we have a $\Theta(1/\eps^4)$-query algorithm from the first section. 

\begin{proposition}
Fix a Hermitian $\AA \in \R^{n \times n}$ with $\|\AA\|_\infty \leq 1$. 
Let $v \in \R^n$ be a unit eigenvector of $\AA$ so that $\AA v = \lambda v$. Then we have the following
\begin{enumerate}
    \item[(a)] $\lambda \leq \|v\|_1^2$
    \item[(b)] $\|v\|_\infty \leq \frac{\sqrt{n}}{|\lambda|}$ 
    \item[(c)] $\|v\|_4^4 \leq\frac{n}{|\lambda|^2}$
    \item[(d)] $\|\lambda v v^T\|_4 \leq \sqrt{n}$
      \item[(e)] $\|(\lambda v v^T)_{i,*}\|_2 \leq \sqrt{n}$ for any $i \in [n]$. 
\end{enumerate}
\end{proposition} 
\begin{proof}
For $(a)$, we have $\lambda = v^T \AA v \leq \sum_{i,j} |v_i| |v_j| = \|v\|_1^2$. For $(b)$, for any $j$ we have $|v_j| = |\lambda^{-1} \langle \AA_{j,*}, v \rangle |\leq |\lambda^{-1}| \|\AA_{j,*}\|_2 \leq \frac{\sqrt{n}}{|\lambda|}$.  Using $(b)$ and the fact that $\|v\|_2 =1$, we know that $\|v\|_4^4$ is maximized by having equal $\frac{|\lambda|^2}{n}$ coordinates equal to $\frac{\sqrt{n}}{|\lambda|}$, which gives $\|v\|_4^4 \leq \frac{n}{|\lambda|^2}$, demonstrating $(c)$. 
For $(d)$, we have $\|\lambda v v^T\|_4^4 = \sum_{i,j} \lambda^4 v_i^4 v_j^4 = \lambda^4 \|v\|_4^8 \leq \lambda^4 \frac{n^2}{|\lambda|^4} \leq n^2$ again using $(b)$. Finally, for $(e)$, we have $\|(\lambda v v^T)_{i,*}\|_2^2 = \sum_j \lambda^2 v_i^2 v_j^2 = \lambda^2 v_i^2 \leq n$ using $(b)$. 
\end{proof}

Now decompose $\AA = \BB + \LL$ where $\BB = \sum_{i : \lambda_i > C \eps^2 n} \lambda_i v_i v_i^T$, for some constant $C$ that we will later choose. Notice that $|\{i : \lambda_i > C \eps^2 n\}| \leq \frac{1}{(C \eps^2)^2}$, since we have $\sum_i \lambda_i^2 \leq n^2$.  
Note that $|\BB_{p,q}| = |\sum_{i : \lambda_i > C \eps^2 n} \lambda_i (v_{i})_p(v_{i})_q| \leq \sum_{i : \lambda_i > C \eps^2 n}\frac{n}{\lambda_i} \leq \frac{1}{(C \eps^2)^3 }$, thus $\|\BB\|_\infty \leq \frac{1}{(C\eps^2)^3}$. Since $\|\AA\|_\infty \leq 1$, we also have $\|\LL\|_\infty \leq \frac{1}{(C\eps^2)^3} + 1$. Moreover, by the prior proposition and the triangle inequality, we have 
\[\|\BB\|_4 \leq \sum_{i : \lambda_i > C \eps^2 n} \|\lambda_i v_{i}v_{i}^T \|_4 \leq \frac{\sqrt{n}}{(C \eps^2)^2} \]
Or $\|\BB\|_4^4 \leq  \frac{n^2}{(C \eps^2)^8}$. 
Moreover, we have $$\|\BB_{j,*}\|_2  \leq  \sum_{i : \lambda_i > C \eps^2 n}  \|\lambda_i (v_i v_i^T)_{j,*}\|_2 \leq \frac{\sqrt{n}}{(C \eps^2)^2}$$
So $\sum_j \|\BB_{j,*}\|_2^4 \leq \frac{n^3}{(C \eps^2)^8}$. 
Thus, we can apply Lemma \ref{lem:samplefrob} with $c_1 = c_2 = \frac{1}{(c \eps^2)^8}$ on the matrix $\BB$. Thus setting $k = \Theta(\frac{1}{\eps^{18}})$ yields the following:


\rajesh{The bound on $\sum_j \|\BB_{j,*}\|_2^4 $ can be improved to $n^3$ using that $B,L$ have ortho columns and rows, and must sum to vectors with norm $\sqrt{n}$.}

\rajesh{Maybe apply this arguement to preserve norm of $L$, then use inverse Lidskii's?}

\begin{lemma}
   Fix any constant $\delta > 0$, and suppose $\AA$ is $\eps$-far from PSD. Decompose $\AA = \BB + \LL$ as above, Let $S \subset [n]$ be a random subset of expected size $k = \Theta(\frac{1}{\eps^{18} })$. Then with probability $1-\delta$, we have simultaneously:
   \begin{enumerate}
       \item $\|\AA_{S \times S}\|_F^2 =  \alpha k^2 \pm \eps  k^2 / 1000$
       \item  $\|\BB_{S \times S}\|_F^2 \leq(\alpha - \eps) k^2 + \pm \eps k^2 / 1000$.
   \end{enumerate}
   \end{lemma}
   \noindent
   We will also need the following proposition.
   \begin{proposition}[PSD matrices are top heavy]\label{prop:topheavy}
   Let $\DD \in \R^{k \times k}$ be such that $\|\DD\|_\infty \leq 1$, and let $\lambda_1(\DD) \geq \lambda_2(\DD) \geq \dots \geq \lambda_k(\DD)$ be its eigenvalues. Then if $\DD$ is PSD, we have
   \[\sum_{i \leq t}\lambda_i(\DD)^2 \geq \|\DD\|_F^2 - t^{-1} k^2\] 
   for any $t \in [k]$.
   \end{proposition}
\begin{proof}
We first show that $\lambda_t(\DD) \leq t^{-1} k$. To see this, suppose $\lambda_{t}(\DD) > t^{-1} k$. Then because $\DD$ is PSD, we would have $\sum_i \lambda_i >t \cdot t^{-1} k = k$, which contradicts the fact that $\sum_{i > t} \lambda_i(\DD) \leq \text{Tr}(\DD) \leq k $ following from the bound $\|\DD\|_\infty \leq 1$. Thus, $\lambda_{t}(\DD) \leq t^{-1} k$. Using this and the bound on $\sum_{i > t} \lambda_i(\DD)$, it follows that the quantity $\sum_{i > t} \lambda_i(\DD)^2$ is maximimized by having $t $ eigenvalues equal to $t^{-1} k$, yielding $\sum_{i > t} \lambda_i(\DD)^2 \leq t^{-1} k^2 $. Thus, if it were also that case that $\sum_{i \leq t}\lambda_i(\DD)^2 < |\DD\|_F^2 - t^{-1} k^2$ then we would have $\sum_i \lambda_i(\DD) < |\DD\|_F^2 - t^{-1} k^2 + t^{-1} k^2 = \|\DD\|_F^2$, which is a contradiction because  $\sum_i \lambda_i(\DD) = \|\DD\|_F^2$, which completes the proof.
\end{proof}

  \begin{proposition}\label{prop:nottopheavy}
   Let $\DD \in \R^{k \times k}$ be such that $\|\DD\|_\infty \leq 1$, and let $\lambda_1(\DD) \geq \lambda_2(\DD) \geq \dots \geq \lambda_k(\DD)$ be its eigenvalues.   Let $\sigma:[n] \to [n]$ denote the re-ordering of the eigenvalues by magnitude, so that $|\lambda_{\sigma(1)} | \geq |\lambda_{\sigma(2)}| \geq \dots \geq |\lambda_{\sigma(k)}|$. Fix any $t \geq 1$. Suppose $\DD$ is at least $(1/t)$-far in $L_2$ from PSD, so that $\sum_{i : \lambda_i(\DD) < 0} \lambda_i^2(\DD) \geq   k^2/t$, and suppose further that $\lambda_k(\DD) > - \frac{k}{2t}$. Then we have
   \[\sum_{i \leq t}\lambda_{\sigma(i)}(\DD)^2 < \|\DD\|_F^2 - t^{-1} k^2/2\] 
   for any $t \in [k]$.
   \end{proposition}
   \begin{proof}
  Let $W \subseteq [n]$ be the set of values $i \in [n]$ such that $\lambda_{\sigma(i)} < 0$. By assumption: $\sum_{i \in W} \lambda_{\sigma(i)}^2 \geq \ n^2$, and moreover $\max_{ i \in W} |\lambda_{\sigma(i)}| \leq \frac{k}{2t}$.  Now note that
   \[\sum_{i \in W} \lambda_{\sigma(i)}^2 = \sum_{i \in W, i \leq t} \lambda_{\sigma(i)}^2 + \sum_{i \in W, i > t} \lambda_{\sigma(i)}^2\]
 By the $\ell_\infty$ bound on the negative eigenvalues, we have that  $ \sum_{i \in W, i \leq t} \lambda_{\sigma(i)}^2 \leq t ( \frac{k}{2t})^2 = k^2 / 4t$. Thus we must have $\sum_{i \in W, i > t} \lambda_{\sigma(i)}^2 \geq (3/4)k^2/t$, giving
   
   \begin{equation}
       \begin{split}
           \sum_{i > t} \lambda_{\sigma(i)}^2  & \geq \sum_{i \in W, i > t} \lambda_{\sigma(i)}^2 \\
           & \geq (3/4)k^2/t \\
       \end{split}
   \end{equation}
   Since $\|\DD\|_F^2 =   \sum_{i \leq t} \lambda_{\sigma(i)}^2  +  \sum_{i > t} \lambda_{\sigma(i)}^2$, it follows that $ \sum_{i \leq t} \lambda_{\sigma(i)}^2  \leq \|\DD\|_F^2 -(3/4)k^2/t$, as needed. 
   
   \end{proof}
   

\begin{theorem}
Let $\AA \in \R^{n \times n}$ be Hermitian matrix with $\|\AA\|_\infty \leq 1$ that is $\eps$-far from PSD in $L_2$. Then if $S \subset [n]$ is a random subset with expected size $k = \Theta(\frac{\log(n)}{\eps^{18} })$, we have that $\AA_{S \times S}$ is not PSD with probability at least $2/3$.
\end{theorem}
\begin{proof}
First condition on the prior Lemma holding with probability $1-\delta$ for a sufficiently small constant $\delta$.  We now claim that $\|\LL_{S \times S}\| \leq \eps^2 k/1000$, after setting the constant $C>0$ to be sufficiently small, with probability at least $99/100$. This will follow directly from Theorem \ref{thm:tropp}, setting $\delta = \frac{k}{n}$ with $p=2$. To see this, note that the first term can be bounded by $O(\log(n) \|\LL\|_\infty) =O( \log(n) (\|\BB\|_\infty +1) ) = O(\frac{\log n}{ \eps^6})$. The second term can be bounded by $O(\frac{k}{\sqrt{n}}  \sqrt{\log(n)} \|\LL\|_\infty ) \leq O(\frac{k}{\sqrt{n}\eps^6} \sqrt{\log(n)})$. The third term can be bounded by $\frac{k}{n}\|\LL\| \leq   C \eps^2 k $. Since $\RR \DD \RR$ is a diagonal matrix, the final term can be bounded by $O( \|\LL\|_\infty) = O( \frac{1}{\eps^6})$. Altogether, we have
\[  \mathbb{E}_2 \|\LL_{S \times S}\| \lesssim \frac{\log(n) }{\eps^6} + \frac{k \sqrt{\log(n)} }{n^{1/2}\eps^6} + C\eps^2 k  \] 
Note that if $k \geq n$, then we are reading the whole matrix anyway, so $k/\sqrt{n} \leq \sqrt{k}$. Setting $k \gtrsim C^{-2}  \frac{\log(n)}{\eps^{16}}$ large enough, the final term dominates up to any arbitrarily large constant factor, and by Markovs we obtain $\|\LL_{S \times S}\| \leq \eps^2 k/1000$ with probability $99/100$ after taking $C$ small enough. 

By the min-max principle, we now have $\lambda_i(\AA_{S \times S}) = \lambda_i(\BB_{S \times S}) \pm \|\LL_{S \times S}\| = \lambda_i(\BB_{S \times S}) \pm \eps^2 k/1000$ for every $i \in [|S|]$. Now set $t= 100/\eps$, and observe:
\begin{equation}
    \begin{split}
        \sum_{i \leq t} \lambda_i(\AA_{S \times S})^2 &\leq \sum_{i \leq t} (\lambda_i(\BB_{S \times S}) + \eps^2 k /1000)^2 \\
        &\leq \|\BB_{S \times S}\|_F^2 + t \eps^2 k^2/1000  + t \eps^4 k^2 / 1000^2\\ &\leq \|\BB_{S \times S}\|_F^2 +  \eps k^2/5 \\
    \end{split}
\end{equation}
 Now condition on the prior Lemma, we have that $\|\BB_{S \times S}\|_F^2 \leq (\alpha - \eps)k^2 + \eps k^2 / 1000$ and $\|\AA_{S \times S}\|_F^2 \geq \alpha k^2 - \eps k^2/1000$, thus  $\|\BB_{S \times S}\|_F^2 \leq \|\AA_{S \times S}\|_F^2  - \eps k^2(1 -1/500)$,  which yields: 
\begin{equation}\label{eqn:topbound}
    \begin{split}
\sum_{i \leq t} \lambda_i(\AA_{S \times S})^2 &\leq \|\BB_{S \times S}\|_F^2 + \eps k^2 / 5 \\
&< \|\AA_{S \times S}\|_F^2  - \frac{3}{4}\eps k^2 \\
    \end{split}
\end{equation}
But we can now apply Proposition \ref{prop:topheavy} with the same $t = 100/\eps$ as above, using the fact that $|S| < 2k$ with probability at least $99/100$, which implies that if $\AA_{S \times S}$ was PSD then we would have $\sum_{i \leq t} \lambda_i(\AA_{S \times S})^2 \geq \|\AA_{S \times S}\|_F^2  -  \eps k^2 / 50$. But this contradicts the upper bound of Equation \ref{eqn:topbound}, which completes the proof of the Theorem after union bounding over all condition upon events which held with large constant probability. 

\end{proof}

%\TODO{Generalize above proofs to any $\alpha$}

\begin{theorem}
Fix a Hermitian matrix $\AA \in \R^{n \times n}$ with $\|\AA\|_\infty \leq 1$, and suppose we are given the promise that either $(1)$ $\AA$ is PSD or $(2)$ $\AA$ is $\eps$-far in $L_2$ from PSD, meaning $\sum_{i : \lambda_i(\AA) < 0} \lambda_i(\AA)^2 \geq \eps n^2$. Then there is a algorithm which makes at most  $O(\frac{\log^2(n)}{\eps^{36}})$-queries to $\AA$  and determines with probability at least $3/4$ whether $\AA$ is PSD or $\eps$-far in $L_2$ from PSD.
\end{theorem}
\begin{proof}
Follows form last theorem since query complexity is $k^2$.
\end{proof}


 %%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}

\begin{algorithm}[!h]
	\SetKwInOut{Input}{Input}
	\caption{Test PSDNess \label{alg:L2}}
       $k \leftarrow O(\frac{1}{\eps^{2.5}})$\\
       $M \leftarrow O(1/\eps)$\\
    \For{$i=1,2,\dots,M$}{Sample a random subset $S \subset [n]$ of expected size $\ex{|S|} = k$. \\
    	Query $Z^i = A_{S \times S}$. \\
    	\If{$Z^i$ is Not PSD}{
    		
    		\Return{Not PSD}
    	}
    }
\If{If no non-PSD matrix was found}{
\Return{PSD}}
    
\end{algorithm}
Let $Z^+,Z^-$ be the restriction of $A^+,A^-$ to the principle submatrix $S \times S$. Then we can write $Z^+ = \sum_{i> t} \lambda_i (v_i)_S (v_i)^T_S$,  $Z^- = \sum_{i\leq t} \lambda_i (v_i)_S (v_i)^T_S$. Therefore $Z^+$ is PSD and $Z^-$ is NSD. 
We first prove the following anti-concentration Lemma for the Frobenius mass in $A^-$.

\begin{lemma}
   Suppose $x = y + z \in \R^{n}$, where $\|x\|_\infty \leq 1$ and $\langle y,z \rangle = 0$. Then $\|y\|_2^2 \leq n$ and $\|z\|_2^2 \leq n$. Moreover, if we define $y' \in \R^n$ via
   \[   y_i' = \begin{cases} y_i & \text{ if } |y_i| < 4 \\ 0 & \text{ otherwise} \\ \end{cases} \]
   and similarly define $z'$, then $\|y'\|_2^2 \geq \frac{\|y\|_2^4}{n}$ and $\|z'\|_2^2 \geq \frac{\|z\|_2^4}{n}$. 
\end{lemma}
\begin{proof}
  We have $0 \leq  \langle y,z \rangle = \langle x-z,z \rangle = \langle x,z \rangle - \|z\|_2^2 \leq \sqrt{n} \|z\|_2- \|z\|_2^2$, thus $\|z\|_2 \leq \sqrt{n}$ as needed, and the remainder follows by symmetry. 
  
  Now suppose there existed some set $S \subset [n]$ with $|S| < \|z\|_2^2/4$ with $\|z_S\|_2^2 > (1- \frac{\|z\|_2^2}{100n}) \|z\|_2^2$. Then $\|z_{-S}\|_2 \leq \frac{\|z\|_2^2}{10n^{1/2}}$, and we have 
  \begin{equation}
      \begin{split}
       |z\|_2^2 &= \langle x,z \rangle  \\
       &= \langle x,z_{S}  + z_{-S}\rangle \\
       &\leq \sqrt{|S|} \|z\|_2 + \|z_{-S}\|_2 \|x\|_2   \\ 
       & \leq \frac{1}{2}\|z\|_2^2 +  \frac{\|z\|_2^2}{10} \\
       & < \|z\|_2^2 \\
      \end{split}
  \end{equation}
  which is a contradiction. It follows that no such set $S$ with both $|S| < \|z\|_2^2/4$ and $\|z_S\|_2^2 > (1- \frac{\|z\|_2^2}{100n}) \|z\|_2^2$ can exist. Now let $S$ be the set of $i \in [n]$ such that $z_i > 4$. Clearly $|S| \leq \|z\|_2^2 / 16$, thus by the above, it follows that $\|z'\|_2^2 = \|z_{-S}\|_2^2 \geq \frac{\|z\|_2^4}{n}$.  
 
\end{proof}



\begin{corollary}\label{cor:decomp}
   Decompose $A = A^+ - A^-$ as above. Let $D \in \R^{n \times n}$ be the matrix defined by \[   D_{i,j} = \begin{cases} A^-_{i,j} & \text{ if } |A^-_{i,j}| < 4 \\ 0 & \text{ otherwise} \\ \end{cases} \]
   Then $\|D\|_2^2 \geq  \eps^2 n^2$
\end{corollary}
\begin{proof}
 By relationships of $p$-norms, we have $\|D\|_f^2\geq  \frac{1}{n}\sum_i\|A_{i,*}^-\|_2^4 \geq \frac{1}{n^2}(\sum_i\|A_{i,*}^-\|_2^2)^2 = n^{-2} \|A^-\|_F^4 \geq \eps^2 n^2$. 
\end{proof}
 
 
 
 \begin{proposition}
 If $A$ is PSD, and $S \subseteq [n]$ is a random sample of size $|S| = k =O(1/\eps^2)$, then $\|(A_S)_{-t}\|_F^2 \leq \eps^2 k^2/5$ with probability $9/10$, where $t = O(1/\eps^2)$ and $(A_S)_{-t}$ is $A_S$ projected away from the top $t$ singular values of $A_S$. 
 \end{proposition}
 \begin{proof}
  Let $Z_{t}$ and $Z_{-t}$ be the restrictions of $A_{t}$ and $A_{-t}$. First note that $A_{-t}$ can have no singular values larger than $\eps^2 n/100$, since this would imply that more than $t$ eigenvectors of $A$ are above this threshold, which would violate the fact that Tr$(A) \leq n$. It follows that $\|A_{-t}\|_F^2 \leq (\eps^2/100) n^2$.
  
  
   Thus $\ex{\|Z_{-t}\|_2^2} \leq k + \eps^2 k^2/100 \leq \eps^2 k^2 / 50$. By Markov's, we have $\|Z_{-t}\|_2^2 \leq  \eps^2 k^2/5$ with probability $9/10$. Since $Z = Z_t + Z_{-t}$, and $Z_t$ has rank at most $t$, projecting away from the top $t$ coordinates can only result in a norm at most $\|Z_{-t}\|_2 \leq  \eps^2 k^2/5$.  
   \end{proof}
 
 
\end{comment}
 
 
 %%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%
 
 
% \subsection{A possibly useful lemma for the future}
%  \begin{lemma}
%  	Suppose $\sum_i (A_{i,i}^+)^2 \leq C n$ for some $C>0$. 
%  	Them if $A$ is not PSD, and $S \subseteq [n]$ is a random sample of size $|S| = O(\frac{C}{\eps})$, then $A_S = A_{S \times S}$ is not PSD with probability at least $\Omega(\eps)$. 
 	
%  \end{lemma}
% \begin{proof}
% We have $Z = Z^+ + Z^{-}$, where $Z^+ = A^+_{S \times S}$, $Z^- = A^-_{S \times S}$.  Consider the random variable $X_S  = \sum_{i j} \delta_i \delta_j\left( A_{i,j}^2 - (A_{i,j}^+)^2\right)$.  Note that 
% \begin{equation}
%     \begin{split}
%         \ex{X_S} & = \frac{k^2}{n^2}\left(\sum_{i \neq j} A_{i,j}^2 - (A_{i,j}^+)^2  \right) + \frac{k}{n}\left(\sum_i A_{i,i}^2 - (A_{i,i}^+)^2	\right)  \\
%         & \geq \frac{k^2}{n^2}\left( \|A\|_F^2 - n - \sum_{i \neq j}  (A_{i,j}^+)^2  \right) - Ck   \\
%         & = \frac{k^2}{n^2}\left( \|A^+\|_F^2 + \|A^-\|_F^2 - n - \sum_{i \neq j}  (A_{i,j}^+)^2  \right)- Ck  \\
%          & = \frac{k^2}{n^2}\left( \sum_{i} (A_{i,i}^+)^2+ \|A^-\|_F^2 - n   \right)- Ck  \\
%           & \geq \frac{k^2}{n^2}\left( \|A^-\|_F^2 - n  \right)- Ck  \\
%           & \geq \eps k^2  - \frac{k^2}{n} - Ck   \\
%             & \geq \eps k^2/2   \\
%     \end{split}
% \end{equation}
% Where in the last inequality, we used the fact that if $\eps < 4/n$, then we can read the whole matrix in $O(1/\eps^2)$ total queries. 
% Now consider $\pr{X_S < \eps k^2/4}$. Observe that $X_{S} \leq k^2$ deterministically, since $X_S \leq \|Z\|_F^2 = \|A_{S\times S}\|_F^2 \leq k^2$. So we have $\ex{X_S} \leq k^2 \pr{X_S > \eps k^2 /4} +(\eps k^2 /4) \pr{X_S \leq \eps k^2 /4}$. Thus
% \begin{equation}
%     \begin{split}
%         \pr{X_S > \eps k^2/4} &\geq  \frac{\ex{X_S} - (\eps k^2 /4) \pr{X_S \leq \eps k^2 /4}}{k^2} \\
%          &\geq  \frac{\ex{X_S} - (\eps k^2 /4) }{k^2} \\
%           &\geq  \eps /4 \\
%             \end{split}
% \end{equation}
% Let $\mathcal{E}$ be the event that $X_S > \eps k^2/4$. Conditioned on $\mathcal{E}$, we have
% \[\|Z\|_F^2 > \|Z^+\|_2^2 + \eps k^2/4	\]
% It follows that $Z$ is not PSD, because $Z = Z^+ + Z^-$, and $Z^-$ is NSD, and $Z$ has strictly larger norm than $Z^+$. To see this, note that adding an NSD matrix can only decrease each eigenvalue. This can be seen easily from the Rayleigh quotient and min-max principle: which gives $x Z^+ x \leq xZ^+ x - x Z^- x$ for all $x$. Thus, for the norm increases after adding an NSD matrix, one of the eigenvalues must now be negative, which completes the proof. 
% \end{proof}



==> Sketching.tex <==
%!TEX root = ../main.tex


\section{Sketching $L_2$ Gap}
\TODO{Lower bounds for spectral sketching imply lower bounds for sketching PSD gap -- just test if $\lambda I - A$ is PSD for different $\lambda$. Use a $c\eps n $-approx of spectral norm for large $c$ to reduce to $O(1)$ choices of $\lambda$, giving $1/\eps^2$ lower bound}


\TODO{Can try subtracting off diagonal. This makes PSD case not PSD, but still keeps a gap between the cases. Then show that this gap can be estimated.}

Let $A \in \R^{n \times n}$ be a symmetric matrix with eigenvectors $v_1,v_2,\dots,v_m$, for $m \leq n$, and eigenvalues $\lambda_1 \leq \lambda_2 \leq \dots \leq \lambda_k < 0 \leq \lambda_{k+1} \leq \dots \leq \lambda_m$. Note that $\|A\|_F^2 = \sum_{i=1}^m \lambda_i^2$. Now let $\eps = \frac{ \sum_{i=1}^k \lambda_i^2}{\|A\|_F^2} \leq 1$, which is a measure of the fraction of $A$ that is negative. We consider the sensing model, where the algorithm fixes sensing matrices $X_1,\dots,X_\ell \in \R^{n \times n}$ and observes $\rho_i \langle \text{vec}(X_i), \text{vec}(A) \rangle = \text{Tr}(X_i^T A)$. Thus the observation $\rho_i$ is a linear function of the enties of $A$. 




\begin{proposition}
Let $A \in \R^{n \times n}$ be any fixed matrix. Then if  $G \in \R^{t \times n}$ is a i.i.d. matrix of Gaussians scaled by $1/\sqrt{t}$, where $t = \Omega(1/\eps)$, then 
\[  \|G\left(A \right)G^T - \frac{\text{Tr}(A) + 10 \alpha \|A\|_F}{t} \mathbb{I}_t\|_F^2 = (1 \pm \eps) \|A\|_F^2 \]    
with probability...
\end{proposition}
\begin{proof}
Write $A = Q \Lambda Q^T$ as the eigendecomposition. Note that $G Q \in \R^{t \times }$ is distributed again as i.i.d. Gaussians scaled by $1/\sqrt{t}$. Thus we can consider the matrix $G\Lambda G^T$.

First, if $i \neq j$, we have $\ex{ (G\Lambda G^T)_{i,j}^2}= \ex{ \left( \sum_k G_{i,k} G_{j,k} \lambda_k(A) \right)^2 } = t^{-2}\sum_k  \lambda_k(A)^2 = \|A\|_F^2/t^2$. \textbf{Compute Variance of off-diagonal and show concentration}.


Next, if $i=j$, 
$(G \Lambda G^T)_{i,i} = \sum_k G_{i,k}^2 \lambda_k$. Now let $X_k =h_k^2 \lambda_k - \lambda_k$, where $h_k \sim \mathcal{N}(0,1)$ and note $\ex{X_k} = 0$. Note moreover that $|X_k| \leq \|A\|_2 \leq \|A\|_F$ deterministically. Thus by Bernstein's inequality:

\begin{equation}
    \begin{split}
    \bpr{  |\sum_k h_k^2 \lambda_k- \text{Tr}(A)| > \alpha \|A\|_F } &\leq \exp\left( \frac{\frac{1}{2}\alpha^2 \|A\||_F^2 }{\sum_{k=1}^n \ex{X_i^2} + \frac{\alpha}{3}\|A\|_F^2 }\right)    \\
&\leq \exp\left( \frac{\frac{1}{2}\alpha^2 \|A\||_F^2 }{\|A\|_F^2 + \frac{\alpha}{3}\|A\|_F^2 }\right)    \\
&\leq \exp\left( \alpha / 3\right)    \\
    \end{split}
\end{equation}
Setting $\alpha = \Theta(\log(t))$, we have that $(GAG)_{i,i} =\left( \text{Tr}(A) \pm O(\log(n)) \|A\|_F\right)t^{-1}$ for all $i \in [t]$ with probability $1-1/\poly(t)$. Since the diagonal is a $1/t$ fraction of the whole matric, it follows that 
\[  \|G\left(A \right)G^T - \frac{\text{Tr}(A) + 10 \alpha \|A\|_F}{t} \mathbb{I}_t\|_F^2 = (1 \pm \eps) \|A\|_F^2 \]    

\end{proof}
\textbf{Matrix Chernoff for completeness, Bernsteins and losing $L_2$ mass for soundness}\\

\begin{lemma}
If $A$ is PSD, we have 
\[\lambda_{\min}(GAG^T) \geq \sum_i \lambda_i(A) = \text{Tr}(A) - 10 \|A\|_F \] with probability $1-\exp(\Omega(\sum_i \lambda_i(A) ))$, where $G \in \R^{t \times n}$ is i.i.d. Gaussian. 
\end{lemma}
\begin{proof}
We can write $GAG^T = G\Lambda G^T = \sum_{i=1}^n G_i \lambda_i G_i^T$, where $G_i \in \R^t$ is the $i$-th column of $G$. Let $X_i = G_i \lambda_i G_i^T$. Note that $\ex{\sum_i X_i} = \text{Tr}(A) \mathbb{I}_n$, so $\mu_{\min} = \lambda_{\min} \left(\ex{\sum_i X_i  }\right) =\text{Tr}(A)$. Moreover, we can condition on the fact that $\|G_i\|_2 \leq \sqrt{\log(n)t}$ w.h.p for all $i$ (make this formal to use in Chernoff bound).

Then by matrix chernoff, we have:

%\[  \bpr{\lambda_{\min}(\sum_i X_i) \leq (1 - \frac{\alpha \|A\|_F}{\text{Tr}(A)})\text{Tr}(A)}   } \leq d\exp\left(  \frac{\alpha^2 \|A\|_F^2}{\text{Tr}(A)} \frac{1}{2\sqrt{\log(n)t}}  \right)\]    
\end{proof}

\textbf{Rest of proof:} Compute $GAG^T$, if $A$ is not PSD then  $A = A^+ + A^-$ and $\|GAG^T\|_F^2 >\|GA^+G^T\|_F^2$ since both are preserved so $GAG^T$ is not PSD.


\newpage

First, we restate a result of \cite{andoni2013eigenvalues}.
\begin{theorem}[Theorem 1.3 \cite{andoni2013eigenvalues}] 
Fix $\eps>0$ and let $A \in \R^{n \times m}$ be any matrix with singular values $\sigma_1 \geq \sigma_2 \geq \dots \geq \sigma_{\min\{m,n\}}$. Then there is a linear sketch of the matrix $A$ using space $O(k\eps^{6}\log(1/\delta))$ from which one can compute a value $R$ such that with probability $1-\delta$
\[  R = (1 \pm \eps) \sum_{i > k} \sigma_i^2 \]
\end{theorem}
\begin{lemma}[Theorem 3.2 \cite{andoni2013eigenvalues}] 
Fix any symmetric matrix $A \in \R^{n \times n}$, and let $G \in \R^{t \times n}$ be a i.i.d. Gaussian matrix with $t = \Theta(k/\eps^2)$. Then 
for $i=1,2,\dots,k$, we have
\[  \lambda_i(GAG^T) = \lambda_i(A)(1 \pm \eps) \pm \lambda_{i+1}(A) \]
\end{lemma}



\section{Multiple Negative Eigenvalues in the Sensing/Sketching model}
Let $A \in \R^{n \times n}$ be a symmetric matrix with eigenvectors $v_1,v_2,\dots,v_m$, for $m \leq n$, and eigenvalues $\lambda_1 \leq \lambda_2 \leq \dots \leq \lambda_k < 0 \leq \lambda_{k+1} \leq \dots \leq \lambda_m$. Note that $\|A\|_F^2 = \sum_{i=1}^m \lambda_i^2$. Now let $\eps = \frac{ \sum_{i=1}^k \lambda_i^2}{\|A\|_F^2} \leq 1$, which is a measure of the fraction of $A$ that is negative. We consider the sensing model, where the algorithm fixes sensing matrices $X_1,\dots,X_\ell \in \R^{n \times n}$ and observes $\rho_i \langle \text{vec}(X_i), \text{vec}(A) \rangle = \text{Tr}(X_i^T A)$. Thus the observation $\rho_i$ is a linear function of the enties of $A$. 

%Let us consider the sketch $S A S^T$, where $S \in \R^{k \times n}$ has entries $S_{i,j} \sim \mathcal{N}(0,1)$. Note that $SA S^T \in \R^{k \times k}$ can be represented by $k^2$ observations $\rho_1,\dots,\rho_{k^2}$.




\begin{lemma}
    Let $g_1,g_2,\dots,g_k \sim \mathcal{N}(0,1)$ and fix $a \in \R^k$ with $\sum_i |a_i| = k$, and let $Z = \sum_{i=1}^k |a_i| g_i^2$. Then for any constant $C  > 0$, there exists a constant $c > 0$ such that
      \[      \bpr{Z < k(1 - \frac{C}{\sqrt{k}})}  \geq c \]
\end{lemma}
\begin{proof}
  Note that the pdf of the variable $Z = \sum_i g_i^2$ is given by 
  $p(x) = \frac{x^{k/2 - 1}e^{-x/2} } { 2^{k/2} (k/2)!}$. Setting $x = k(1-C/\sqrt{k})$, we obtain
 \TODO{Fix: finish analysis to bound by $\Omega(k^{-1/2})$}
  
  \begin{equation}
      \begin{split}
          p( k(1-C/\sqrt{k})) &=   \frac{(k(1-\frac{C}{\sqrt{k}}))^{k/2 - 1}e^{-k(1-C/\sqrt{k})/2} } { 2^{k/2} \gamma(k/2)} \\
          & = \left(\frac{(k(1-\frac{C}{\sqrt{k}}))}{2 e^{1 - C/\sqrt{k} }}\right)^{k/2} (k(1-\frac{C}{\sqrt{k}}))^{-1} \frac{1}{(k/2-1)!}\\
               & \geq \left(\frac{k(1-\frac{C}{\sqrt{k}})}{2 e^{1 - C/\sqrt{k} }}\right)^{k/2}  \frac{(\pi k)^{-1/2}}{k(1-\frac{C}{\sqrt{k}})}\left(\frac{e}{k}\right)^{k/2-1} (1 \pm o(1))\\
                 & = \left(\frac{(1-\frac{C}{\sqrt{k}})}{2e^{ - C/\sqrt{k} }}\right)^{k/2}  \frac{(\pi k)^{-1/2}}{k(1-\frac{C}{\sqrt{k}})} \left(\frac{k}{2e}\right) (1 \pm o(1))\\
                  & = \exp \left(\frac{k}{2}(Ck^{-1/2} - Ck^{-1/2} - C^2k^{-1}/2 + O(k^{-3/2}))  \right) \frac{(\pi k)^{-1/2}}{k(1-\frac{C}{\sqrt{k}})} (1 \pm o(1))\\
                     & = \exp \left(-C^2/4 + O(k^{-1/2}))  \right) \frac{(\pi k)^{-1/2}}{k(1-\frac{C}{\sqrt{k}})} (1 \pm o(1))\\
      \end{split}
  \end{equation}
  
  
\end{proof}

==> ky_fan_decay.tex <==

\section{Upper bounds for Schatten and Ky-Fan norm Estimation}

In this section, we prove a new decay theorems for Schatten and Ky-Fan Norms under random restrictions. 
Our techniques use multiple ideas from functional analysis, such as symmetrization and non-commutative Khintchine Inequalities for all $p$ in $(0,2]$. We begin by defining the generalized Ky-Fan norm:

\begin{definition}
Given a $n \times d$ matrix $\AA$, let $\U \Sig \V^T$ be the SVD of $\AA$. Then, for any $k \in [d]$ and $p \in (0,\infty)$, the $(k,p)$-Ky-Fan norm is given by 
\[
\|\AA\|_{K_{k,p}} = \left(\sum^{k}_{i =1} \sigma^{p}_{i}(\AA)\right)^{1/p}
\]
\end{definition}

\begin{remark}The $(k,p)$-Ky-Fan norm captures as special cases the Frobenius norm, all Schatten-$p$ norms and the Operator norm. 
\end{remark}


We begin by stating our main decay results. We obtain new theorems for the behavior of the $(p,k)$-Ky Fan norm when $p \in \{1,2\}$. For $p=2$, this captures the Frobenius norm of the best rank-$k$ approximation to $\AA$. For $p=1$, and $k=n$, we obtain a decay result for Schatten-$1$. 



\begin{theorem}[$(2,k)$-Ky Fan Decay]
\label{thm:top_k_decay}
Given a $n \times n$ symmetric matrix $\AA$, $k \in [n]$ and let $Q$ be a random subset of $[n]$ such that $\expecf{}{|Q|}= \frac{q}{n}$ and let $\AA_{\mid Q}$ be the matrix obtained by restricting the columns of $\AA$ to the subset indexed by $Q$. Then, for $r\in \mathbb{N}$,
\begin{equation*}
    \expecf{r}{\Norm{\AA_{\mid Q}}_{K_{k,2}}} = \sqrt{\frac{q}{n}} \Norm{\AA}_{K_{k,2}} \pm O\left(  \sqrt{k} \log(k)^{1/2} \expecf{r}{ \Norm{\AA_{\mid Q} }_{1\to 2} }  \right)
\end{equation*}
\end{theorem}


\ainesh{adding the right statement and proof for the above}

\ainesh{Next, we obtain a decay theorem for the standard Ky-Fan norm as well as Schatten-$1$. The key techniques we use here are a symmetrization argument for pseudo-norms and the non-commutative khintchine inequality for $p < 1$. This commentary should go elsewhere. }




\begin{theorem}[$(1,k)$-Ky Fan and Schatten-$1$ Decay]
\label{thm:ky_fan_decay}
Given a $n \times n$ symmetric matrix $\AA$, $k \in [n]$ and let $Q$ be a random subset of $[n]$ such that $\expecf{}{|Q|}= \frac{q}{n}$ and let $\AA_{\mid Q}$ be the matrix obtained by restricting the columns of $\AA$ to the subset indexed by $Q$. Then, for $r\in \mathbb{N}$,
\begin{equation*}
    \expecf{r}{\Norm{\AA_{\mid Q}}_{K_{k,1}}} = 2\sqrt{\frac{q}{n}} \Norm{\AA}_{K_{k,1}} \pm O\left(  k \log(k)^{1/2} \expecf{r}{ \Norm{\AA_{\mid Q} }_{1\to 2} }  \right)
\end{equation*}
\end{theorem}


We begin by recalling the non-commutative Khintchine Inequality, originally discovered by Lust-Picard \cite{lust1986inegalites} and Lust-Picard and Pisier \cite{lust1986inegalites}. We use a sharp bound due to Buchholz \cite{buchholz2001operator}, that was subsequently improved by Oliviera \cite{Oliveira_2010} and restated in Meka and Wigderson (Theorem 5.1): 


\ainesh{put right def of NCKI from gilles  pisier }

\begin{theorem}[Non-Commutative Khintchine Inequality]
\label{thm:non_commutative_khintchine}
Let $\AA = \sum_{i \in [t]} \AA_{(i)}$ be a finite sequence of $n \times n$ PSD matrices and for all $i \in [t]$, $\eta_i$ be a Rademacher random variable. Then, there exists a constant $\Delta$ such that with probability $1- ne^{-\Delta^2}$
\begin{equation*}
     -\Delta \left(\sum_{i\in[t]} \AA_{(i)}\AA^{\top}_{(i)} \right)^{1/2} \preceq \sum_{i\in[t]}\eta_i \AA_{(i)} \preceq \Delta \left(\sum_{i\in[t]} \AA_{(i)}\AA^{\top}_{(i)} \right)^{1/2}
\end{equation*}
\end{theorem}


We also require the following simple fact for $L_{p}$-spaces when $p<1$:
\begin{fact}[Triangle and Reverse Triangle Inequality]
\label{fact:tri}
Given vectors $x, y \in \mathbb{R}^d$, for any $p \in (0,1)$,  $\| x +y \|_p \leq 2^{1/p- 1}(\|x\|_p \pm \|y \|_p)$  and $\|x+y\|^p_p = \|x\|^p_p \pm \|y\|^p_p$.
\end{fact}

% \begin{theorem}[Non-Commutative Khintchine Inequality]
% \label{thm:non_commutative_khintchine}
% Let $\AA = \sum_{i \in [t]} \AA_{(i)}$ be a finite sequence of $n \times n$ matrices and for all $i \in [t]$, $\eta_i$ be a Rademacher random variable. Then, for any $p \in [1,2]$, for all $\X_{(i)} + \Y_{(i)} = \AA_{(i)}$,
% \begin{equation*}
%     \expecf{\eta}{\Norm{\sum_{i\in[t]}\eta_i \AA_{(i)}}_{\cS_p}} \leq \Norm{ \left(\sum_{i\in[t]} \X^{\top}_{(i)}\X_{(i)} \right)^{1/2}}_{\cS_p} + \Norm{\left(\sum_{i\in[t]} \Y_{(i)}\Y^{\top}_{(i)}\right)^{1/2}}_{\cS_p}
% \end{equation*}
% \end{theorem}


Next, we show that classical symmeterization arguments extend to pseudo-norms.  
 
\begin{lemma}[Symmetrization for Norms, \cite{} HDP Book]
Given $n$ i.i.d. mean $0$ random vectors $X_1, X_2, \ldots X_n \in \mathbb{R}^d$, let $\{\eta_i\}_{i\in [n]}$ be $n$ Rademacher random variables. Then, for any norm $\| \|_{K}$,
\[
\expecf{}{\Norm{\sum_{i \in [n]} X_i}_K} \leq 2 \expecf{}{\Norm{\sum_{i \in [n]}  \eta_i X_i }_K}
\]
\end{lemma}

Now, we are ready to prove our theorems.


\begin{proof}[Proof of Theorem \ref{thm:top_k_decay}]
Let $K_{*}$ denote the $(k,2)$-Ky-Fan norm.
For all $i \in [n]$, let $\delta_i$ be indicator random variables for $i \in Q$ and thus $\expecf{}{\delta_i} = \delta= q/n$. Let $\AA_{i}$ denote the $i$-th column of $\AA$. Therefore, $\AA = \sum_{i \in [n]} e_i \otimes \AA_i$ and $\AA_{\mid Q} = \sum_{i \in [n]} \delta_i e_i \otimes \AA_i$, where $e_i$ is the $i$-th standard basis vector. Let $\AA = \U \Lam \U^T$ be the Eigendecomposition of $\AA$. Observe,  
\begin{equation*}
    \Norm{\AA }_{K^*} = \left(\sum_{j \in [k]} \lambda^2_j(\AA)\right)^{1/2} = \Norm{\AA^{\top} \AA}_{K_{(k,1)}} = \Norm{\sum_{i \in [n]} \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{(k,1)}}
\end{equation*}
where the second equality follows from $\AA^T \AA = \U \Lam^2 \U^T$ and the definition of $\|\cdot \|_{K_{(k,1)}}$. Similarly,
\begin{equation*}
    \|\AA_{\mid Q}\|_{K^*}  = \Norm{\sum_{i \in [n]} \delta_i \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{(k,1)}}
\end{equation*}
First, we do the analysis for the expectation. 
We would like to bound $\expecf{}{\Norm{\AA_{\mid Q}}_{K^*}}$ as follows
\begin{equation}
\label{eqn:decay_statement}
\begin{split}
    \expecf{}{\Norm{\AA_{\mid Q}}_{K^*}}^2 &  = \expecf{}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i} +  \delta \AA^{\top}\AA }^{1/2}_{K_{k,1}}} \\
    & = \Norm{ \delta \AA^{\top}\AA }^{1/2}_{K_{k,1}} \pm \expecf{}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{k,1}}}\\
    & = \sqrt{\delta} \Norm{\AA}_{K^*} \pm \expecf{}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{k,1}}}
\end{split}
\end{equation}
where the second equality follows from triangle and reverse triangle inequality on the square-root of the Ky-Fan norm. Observe, we get the rate of decay we desire for $\|\AA\|_{K^*}$ and it suffices to bound the additive term. 
Using Fact \ref{} we know that $K_{k,1}$ is a norm and it follows from Lemma \ref{} that we can bound the expectation by introducing Rademacher random variables $\eta_i$ and observing that $\eta_i(\delta_i - \delta)$ has the same distribution as $\eta_i \delta_i$ and thus 
\begin{equation*}
    \expecf{}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{k,1}}} \leq 2 \expecf{}{\expecf{\eta}{\Norm{ \sum_{i \in [n]} \eta_i \delta_i\AA_{i} \otimes \AA_{i}}_{K_{k,1}}}^{1/2}}
\end{equation*}


Here, we apply Theorem \ref{thm:non_commutative_khintchine} with $\X_i = \AA_i \otimes \AA_i$ and $\Y_i = 0$ to obtain that with probability at least $99/100$, over a fixing of $Q$, 

\begin{equation}
\label{eqn:khintchine}
\begin{split}
    \expecf{\eta}{\Norm{ \sum_{i \in [n]} \eta_i\delta_i \AA_{i} \otimes \AA_{i}}_{K_{k,1}}} 
    %& \leq \expecf{\eta}{\Norm{ \sum_{i \in [n]} \eta_i\delta_i \AA_{i} \otimes \AA_{i}}_{\cS_1}} \\
    & \leq O\left(\sqrt{p }\right) \Norm{\left( \sum_{i \in [n]} \delta_i (\AA_{i} \otimes \AA_{i})^{\top}  \AA_{i} \otimes \AA_{i} \right)^{1/2} }_{K_{k,1}}   \\
    & \leq O\left(\sqrt{p } \right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot \Norm{\AA_{\mid Q} }_{K_{(k,1)}} \\ 
    %& \leq O\left(\sqrt{p }\log(n)\right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot  \sum_{i \in [n]} \Norm{ \delta_i e_i \otimes \AA_i }_{K_{(k,1)}} \\
    %& \leq O\left(\sqrt{p }\log(n)\right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot \Norm{\AA_{\mid Q}}_F 
    & \leq O\left(\sqrt{pk } \right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot \Norm{\AA_{\mid Q} }_{K_{(k,2)}}
\end{split}
\end{equation}
where we incur a $\sqrt{k}$ factor relating $K_{(k,1)}$ to $K_{(k,2)}$.
Plugging this back into Equation \eqref{eqn:decay_statement}, we get 
\begin{equation}
\label{eqn:top_k_bound_for_algo}
    \begin{split}
         \expecf{}{\Norm{\AA_{\mid Q}}_{K^*}} &  = \sqrt{\delta} \Norm{\AA}_{K^*} \pm O\left(\sqrt{pk }\expecf{}{\Norm{\AA_{\mid Q}}_{1\to 2}} \right)^{1/2}  \cdot  \expecf{}{\Norm{\AA_{\mid Q} }_{K_{(k,2)}}}^{1/2}
    \end{split}
\end{equation}
where we used Cauchy-Schwarz. \ainesh{This above bound should suffice for our applications}

\ainesh{unfortunately going from the above to a clean bound incurs }

Now, we are ready to bound the $r$-th moment.
Observe $\expecf{r}{\Norm{\AA_{\mid Q}}_{K^*}}^2 = \expecf{}{\Norm{ \delta_i \AA_i \otimes \AA_i }^{r/2}_{K_{k,1}}}^{2/r}$.
Then,
\begin{equation}
\label{eqn:decay_statement}
\begin{split}
    \expecf{r}{\Norm{\AA_{\mid Q}}_{K^*}}^2 &  = \expecf{}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i} +  \delta \AA^{\top}\AA }^{r/2}_{K_{k,1}}}^{2/r} \\
    & = \Norm{ \delta \AA^{\top}\AA }_{K_{k,1}} \pm \expecf{}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i}}^{r/2}_{K_{k,1}}}^{2/r}\\
    & = \delta \Norm{\AA}^2_{K^*} \pm \expecf{}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i}}^{r/2}_{K_{k,1}}}^{2/r}
\end{split}
\end{equation}
where the second equality follows from triangle and reverse triangle inequality on the Ky-Fan norm then triangle inequality for $\expecf{r/2}{}$. Observe, we get the rate of decay we desire for $\|\AA\|_{K^*}$ and it suffices to bound the additive term. 
Since $K_{k,1}$ it follows from Lemma \ref{} that we can bound the expectation by introducing Rademacher random variables $\eta_i$ and observing that $\eta_i(\delta_i - \delta)$ has the same distribution as $\eta_i \delta_i$ and thus 
\begin{equation*}
    \expecf{}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i}}^{r/2}_{K_{k,1}}} \leq 2 \expecf{}{\expecf{\eta}{\Norm{ \sum_{i \in [n]} \eta_i \delta_i\AA_{i} \otimes \AA_{i}}^{r/2}_{K_{k,1}}}}
\end{equation*}


Here, we apply Theorem \ref{thm:non_commutative_khintchine} with $\X_i = \AA_i \otimes \AA_i$ and $\Y_i = 0$ to obtain that with probability at least $99/100$, over a fixing of $Q$, 

\begin{equation}
\label{eqn:khintchine}
\begin{split}
    \expecf{\eta}{\Norm{ \sum_{i \in [n]} \eta_i\delta_i \AA_{i} \otimes \AA_{i}}_{K_{k,1}}} 
    %& \leq \expecf{\eta}{\Norm{ \sum_{i \in [n]} \eta_i\delta_i \AA_{i} \otimes \AA_{i}}_{\cS_1}} \\
    & \leq O\left(\sqrt{p }\right) \Norm{\left( \sum_{i \in [n]} \delta_i (\AA_{i} \otimes \AA_{i})^{\top}  \AA_{i} \otimes \AA_{i} \right)^{1/2} }_{K_{k,1}}   \\
    & \leq O\left(\sqrt{p } \right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot \Norm{\AA_{\mid Q} }_{K_{(k,1)}} \\ 
    %& \leq O\left(\sqrt{p }\log(n)\right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot  \sum_{i \in [n]} \Norm{ \delta_i e_i \otimes \AA_i }_{K_{(k,1)}} \\
    %& \leq O\left(\sqrt{p }\log(n)\right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot \Norm{\AA_{\mid Q}}_F 
    & \leq O\left(\sqrt{pk } \right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot \Norm{\AA_{\mid Q} }_{K_{(k,2)}}
\end{split}
\end{equation}
where we incur a $\sqrt{k}$ factor relating $K_{(k,1)}$ to $K_{(k,2)}$.
Plugging this back into Equation \eqref{eqn:decay_statement}, we get 
\begin{equation}
\label{eqn:second_ky_fan}
    \begin{split}
         \expecf{r}{\Norm{\AA_{\mid Q}}_{K^*}}^2 &  = \delta \Norm{\AA}^2_{K^*} \pm O\left(\sqrt{pk }\expecf{r}{\Norm{\AA_{\mid Q}}_{1\to 2}} \right)  \cdot  \expecf{r}{\Norm{\AA_{\mid Q} }_{K^*}}
    \end{split}
\end{equation}
where we used Cauchy-Schwarz
Observe, $x^2 \leq a x + b$ implies $x \leq \frac{a + \sqrt{a^2 + 4b}}{2} \leq 2a + \sqrt{b}$ and similarly, $x \geq -2a + \sqrt{b}$ and thus from Eqn \eqref{eqn:second_ky_fan}, 
\begin{equation}
    \expecf{r}{\Norm{\AA_{\mid Q} }_{K^*} }  = \sqrt{\delta} \Norm{\AA}_{K^*} \pm O\left(\sqrt{pk }\log(n)\right) \expecf{r}{\Norm{\AA_{\mid Q} }_{1\to 2}} 
\end{equation}
which completes the proof.
\end{proof}

\ainesh{This above proof is straighforward and does not rquire new symm and the variance bound also works out nicely. }

Next, we prove the decay theorem for $(k,1)$-Ky Fan norms.

\begin{proof}[Proof of Theorem \ref{thm:ky_fan_decay}]
For all $i \in [n]$, let $\delta_i$ be indicator random variables for $i \in Q$ and thus $\expecf{}{\delta_i} = \delta= q/n$. Let $\AA_{i}$ denote the $i$-th column of $\AA$. Therefore, $\AA = \sum_{i \in [n]} e_i \otimes \AA_i$ and $\AA_{\mid Q} = \sum_{i \in [n]} \delta_i e_i \otimes \AA_i$, where $e_i$ is the $i$-th standard basis vector. Let $\AA = \U \Lam \U^T$ be the Eigen-Decomposition of $\AA$. Observe,  
\begin{equation*}
    \Norm{\AA }_{K_{k,1}} = \left(\sum_{j \in [k]} |\lambda_j(\AA)|\right) = \left(\sum_{j \in [k]} \left(\lambda^2_j(\AA)\right)^{1/2}\right)^{1/p} = 
    \Norm{\AA^{\top} \AA}^{1/2}_{K_{(k,1/2)}} = \Norm{\sum_{i \in [n]} \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{(k,1/2)}}
\end{equation*}
where the second equality follows from $\AA^T \AA = \U \Lam^2 \U^T$ and the definition of $\|\cdot \|_{K_{(k,1/2)}}$. Similarly, 
\begin{equation*}
    \|\AA_{\mid Q}\|_{K_{k,1}}  = \Norm{\sum_{i \in [n]} \delta_i \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{(k,1/2)}}
\end{equation*}
We would like to bound $\expecf{}{\Norm{\AA_{\mid Q}}_{K_{k,1}}}$. Observe,
\begin{equation}
\label{eqn:decay_statement}
\begin{split}
    \expecf{}{\Norm{\AA_{\mid Q}}_{K_{k,1}}} &  = \expecf{}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i} +  \delta \AA^{\top}\AA }^{1/2}_{K_{k,1/2}}} \\
    & = \expecf{}{\Norm{ \delta \AA^{\top}\AA }^{1/2}_{K_{k,1/2}} \pm \Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i} }^{1/2}_{K_{k,1/2}}}\\
    & = \Norm{ \delta \AA^{\top}\AA }^{1/2}_{K_{k,1/2}} \pm \expecf{}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{k,1/2}}} \\
    & = \sqrt{\delta} \Norm{\AA}_{K_{k,1}} \pm \expecf{}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{k,1/2}}}
\end{split}
\end{equation}
where the second equality follows from triangle and reverse triangle inequality from Fact \ref{fact:tri} and the third follows from linearity of expectation. 

\ainesh{add a proof of symm.}

Observe, we get the rate of decay we desire for $\|\AA\|_{K_{k,1}}$ and it suffices to bound the additive term. Unfortunately $K_{k,1/2}$ is not a norm



using symmetrization, we can bound the expectation by introducing Rademacher random variables $\eta_i$ and observing that $\eta_i(\delta_i - \delta)$ has the same distribution as $\eta_i \delta_i$ and thus 
\begin{equation*}
    \expecf{}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{k,1/2}}} \leq 4 \expecf{}{\expecf{\eta}{\Norm{ \sum_{i \in [n]} \eta_i \delta_i\AA_{i} \otimes \AA_{i}}_{K_{k,1/2}}}^{1/2}}
\end{equation*}
Here, we apply Theorem \ref{thm:non_commutative_khintchine} with $\X_i = \AA_i \otimes \AA_i$  and $\Delta = \sqrt{k}$, to obtain that with probability at least $1-1/\poly(k)$, for all $\ell \in [n]$,
\begin{equation}
    \left|\lambda_{\ell}\left( \sum_{i\in[t]} \eta_i \AA_{i}\otimes \AA_{i} \right)\right| \leq \log(k)^{1/2} \left|\lambda_{\ell}\left( (\AA \AA^T)^{1/2} \right)\right|
\end{equation}
Observe, $\AA^T \AA = \U \mathbf{\Sigma}^2 \U^T$, where $\Sig$ are the singular values of $\AA$ and therefore $(\AA^T \AA)^{1/2}$ has the same singular values as $\AA$. 
Then, for a fixing of $Q$, 
\begin{equation}
\label{eqn:khintchine}
\begin{split}
    \expecf{\eta}{\Norm{ \sum_{i \in [n]} \eta_i\delta_i \AA_{i} \otimes \AA_{i}}_{K_{k,1/2}}} 
    %& \leq \expecf{\eta}{\Norm{ \sum_{i \in [n]} \eta_i\delta_i \AA_{i} \otimes \AA_{i}}_{\cS_1}} \\
    & \leq O\left(\log(k)^{1/2}\right) \Norm{\left( \sum_{i \in [n]} \delta_i (\AA_{i} \otimes \AA_{i})^{\top}  \AA_{i} \otimes \AA_{i} \right)^{1/2} }_{K_{k,1/2}}   \\
    & \leq O\left(\log(k)^{1/2}\right) \Norm{\Norm{\AA_{\mid Q}}_{1\to 2}  \left( \AA^T_{\mid Q} \AA_{\mid Q} \right)^{1/2} }_{K_{k,1/2}}   \\
    & \leq O\left(\log(k)^{1/2}\right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot \Norm{\AA_{\mid Q} }_{K_{k,1/2}} \\ 
    %& \leq O\left(\sqrt{r }\log(k)^{p/2}\right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot  \sum_{i \in [n]} \Norm{ \delta_i e_i \otimes \AA_i }_{K_{(k,1)}} \\
    %& \leq O\left(\sqrt{r }\log(k)^{p/2}\right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot \Norm{\AA_{\mid Q}}_F 
    & \leq O\left(k\log(k)^{1/2}\right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot \Norm{\AA_{\mid Q} }_{K_{k,1}}
\end{split}
\end{equation}
where we incur a $k$ factor by relating $K_{k,1/2}$-norm to the $K_{k,1}$-norm.
Plugging this back into Equation \eqref{eqn:decay_statement}, we get 
\begin{equation}
\label{eqn:second_ky_fan}
    \begin{split}
         \expecf{}{\Norm{ \AA_{\mid Q} }_{K_{k,1}}} &  = \sqrt{\delta} \Norm{\AA}_{K_{k,1}} \pm O\left(k^{1/2}\log(k)^{1/4}\right) \expecf{}{\Norm{\AA_{\mid Q}}_{1\to 2} \cdot  \Norm{\AA_{\mid Q} }_{K_{k,1}} }^{1/2} \\
         & = \sqrt{\delta} \Norm{\AA}_{K_{k,1}} \pm O\left(k^{1/2}\log(k)^{1/4}\right) \expecf{}{\Norm{\AA_{\mid Q}}_{1\to 2}}^{1/2} \expecf{}{  \Norm{\AA_{\mid Q} }_{K_{(k,1)}}}^{1/2}
    \end{split}
\end{equation}
where we used Cauchy-Schwarz
Observe, $x \leq b+ a\sqrt{x}$ implies \[
x \leq \frac{2b + a^2 +\sqrt{a^2 (a^2 + 4 b)} }{2} = b + \frac{  (1+ \sqrt{1+ 4b/a^2}) a^2 }{2}
\] 
%\nadiia{there's a slight issue here that $b/a^2$ need not be $O(1)$.}
and similarly, $x \geq b - + \frac{  (1+ \sqrt{1+ 4b/a^2}) a^2 }{2}$ and thus from \eqref{eqn:second_ky_fan}, 
\begin{equation}
    \expecf{}{\Norm{\AA_{\mid Q} }_{K_{k,1}} }  = 2\sqrt{\delta} \Norm{\AA}_{K_{k,1}} \pm O\left(k\log(k)^{1/2}\right) \expecf{}{\Norm{\AA_{\mid Q} }_{1\to 2}} 
\end{equation}
which completes the proof for $r= 1$.
% \nadiia{we can bound the moments by a constant times what we need.}
% \ainesh{for our application we only work with the equation before applying Cauchy Schwarz.}
Next, we bound the moments of the norm of a random submatrix, for $r\geq 2$.
% \begin{proof}
% Recall,  
% \begin{equation*}
%     \Norm{\AA }_{K_{k,1}}  = \Norm{\sum_{i \in [n]} \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{(k,1/2)}}
% \end{equation*}
% and
% \begin{equation*}
%     \|\AA_{\mid Q}\|_{K_{k,p}}  = \Norm{\sum_{i \in [n]} \delta_i \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{(k,p/2)}}
% \end{equation*}
% We would like to bound $\expecf{r}{\Norm{\AA_{\mid Q}}_{K_{k,1}}}^2  = \left(\expecf{}{\Norm{\AA_{\mid Q}}^{r}_{K_{k,1}}}\right)^{2/r}$. To this end, observe that 
% \begin{equation}
% \label{eqn:ky_fan_ell_2_to_ell_1}
%     \expecf{r}{\Norm{\AA_{\mid Q}}_{K_{k,1}}}^2 = \expecf{}{\Norm{ \sum_{i \in [n]} \delta_i \AA_{i} \otimes \AA_{i} }^{r/2}_{K_{k,1/2}}}^{2/r}
% \end{equation}
Then, using Fact \ref{fact:tri},
\begin{equation}
\label{eqn:decay_statement}
\begin{split}
    \expecf{r}{\Norm{\AA_{\mid Q}}_{K_{k,1}}}^{2} &  = \expecf{}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i} +  \delta \AA^{\top}\AA }^{r/2}_{K_{k,1/2}}}^{2/r} \\
    & = \expecf{r/2}{ 2 \Norm{ \delta \AA^{\top}\AA }_{K_{k,1/2}} \pm 2 \Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i} }_{K_{k,1/2}}}\\
    & = 2\Norm{ \delta \AA^{\top}\AA }_{K_{k,1/2}} \pm 2
    \expecf{r/2}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i}}_{K_{k,1/2}}} \\
    & = 2\delta \Norm{\AA}^2_{K_{k,1}} \pm 2\expecf{r}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{k,1/2}}}^{2}
\end{split}
\end{equation}

Using symmetrization, we can bound the expectation by introducing Rademacher random variables $\eta_i$ and observing that $\eta_i(\delta_i - \delta)$ has the same distribution as $\eta_i \delta_i$ and thus 
\begin{equation*}
    \expecf{r}{\Norm{ \sum_{i \in [n]} (\delta_i - \delta) \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{k,1/2}}}^{2} \leq 4 \expecf{r}{\expecf{\eta}{\Norm{ \sum_{i \in [n]} \eta_i \delta_i\AA_{i} \otimes \AA_{i}}^{1/2}_{K_{k,1/2}}}}^{2}
\end{equation*}
Here, we apply Theorem \ref{thm:non_commutative_khintchine} with $\X_i = \AA_i \otimes \AA_i$  and $\Delta = \sqrt{k}$, to obtain that for any $p \in (0,2]$, with probability at least $1-1/\poly(k)$, for all $\ell \in [n]$,
\begin{equation}
    \left|\lambda_{\ell}\left( \sum_{i\in[t]} \eta_i \AA_{i}\otimes \AA_{i} \right)\right|^{p} \leq \log(k)^{p/2} \left|\lambda_{\ell}\left( (\AA \AA^T)^{1/2} \right)\right|^{p}
\end{equation}
Observe, $\AA^T \AA = \U \mathbf{\Sigma}^2 \U^T$, where $\Sig$ are the singular values of $\AA$ and therefore $(\AA^T \AA)^{1/2}$ has the same singular values as $\AA$. 
Then, for a fixing of $Q$, setting $p$ above to $1/2$
\begin{equation}
\label{eqn:khintchine}
\begin{split}
    \expecf{\eta}{\Norm{ \sum_{i \in [n]} \eta_i\delta_i \AA_{i} \otimes \AA_{i}}^{1/2}_{K_{k,1/2}}} 
    %& \leq \expecf{\eta}{\Norm{ \sum_{i \in [n]} \eta_i\delta_i \AA_{i} \otimes \AA_{i}}_{\cS_1}} \\
    & \leq O\left(\log(k)^{1/4}\right) \Norm{\left( \sum_{i \in [n]} \delta_i (\AA_{i} \otimes \AA_{i})^{\top}  \AA_{i} \otimes \AA_{i} \right)^{1/2} }^{1/2}_{K_{k,1/2}}   \\
    & \leq O\left(\log(k)^{1/4}\right) \Norm{\Norm{\AA_{\mid Q}}_{1\to 2}  \left( \AA^T_{\mid Q} \AA_{\mid Q} \right)^{1/2} }^{1/2}_{K_{k,1/2}}   \\
    & \leq O\left(\log(k)^{1/4}\right) \Norm{\AA_{\mid Q}}^{1/2}_{1\to 2} \cdot \Norm{\AA_{\mid Q} }^{1/2}_{K_{k,1/2}} \\ 
    %& \leq O\left(\sqrt{r }\log(k)^{p/2}\right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot  \sum_{i \in [n]} \Norm{ \delta_i e_i \otimes \AA_i }_{K_{(k,1)}} \\
    %& \leq O\left(\sqrt{r }\log(k)^{p/2}\right) \Norm{\AA_{\mid Q}}_{1\to 2} \cdot \Norm{\AA_{\mid Q}}_F 
    & \leq O\left(\sqrt{k} \log(k)^{1/4}\right) \Norm{\AA_{\mid Q}}^{1/2}_{1\to 2} \cdot \Norm{\AA_{\mid Q} }^{1/2}_{K_{k,1}}
\end{split}
\end{equation}
where we incur a $k$ factor by relating $(1/2)$-norm to the $1$-norm.
Plugging this back into Equation \eqref{eqn:decay_statement}, we get 
\begin{equation}
\label{eqn:second_ky_fan}
    \begin{split}
         \expecf{r}{\Norm{ \AA_{\mid Q} }_{K_{k,1}}}^{2} &  = 2 \delta \Norm{\AA}^2_{K_{k,1}} \pm O\left(k\log(k)^{1/2}\right) \expecf{}{\Norm{\AA_{\mid Q}}^{r/2}_{1\to 2} \cdot  \Norm{\AA_{\mid Q} }^{r/2}_{K_{(k,1)}} }^{2/r} \\
         &  = 2 \delta \Norm{\AA}^2_{K_{k,1}} \pm O\left(k\log(k)^{1/2}\right) \expecf{}{\Norm{\AA_{\mid Q}}^{r}_{1\to 2} \cdot  \Norm{\AA_{\mid Q} }^{r}_{K_{(k,1)}} }^{1\textbf{}/r} \\
         & = 2\delta \Norm{\AA}^2_{K_{k,1}} \pm O\left(k\log(k)^{1/2}\right) \expecf{r}{\Norm{\AA_{\mid Q}}_{1\to 2}} \expecf{r}{  \Norm{\AA_{\mid Q} }_{K_{(k,1)}}}
    \end{split}
\end{equation}
where we used Jensen's in the first equality and Cauchy-Schwarz in the second.
Observe, $x^2 \leq a x + b$ implies $x \leq \frac{a + \sqrt{a^2 + 4b}}{2} \leq a + \sqrt{b}$ and similarlet, $x \geq -a + \sqrt{b}$ and thus from \eqref{eqn:second_ky_fan}, 
\begin{equation}
    \expecf{r}{\Norm{\AA_{\mid Q} }_{K_{k,1}} }  = \sqrt{2\delta} \Norm{\AA}_{K_{k,1}} \pm O\left(k\log(k)^{1/2}\right) \expecf{r}{\Norm{\AA_{\mid Q} }_{1\to 2}} 
\end{equation}
which completes the proof.
\end{proof}


\subsection{Testing Norms in the Bounded Entry Model}

In this subsection, we describe how to obtain estimators for matrix norms from the general decay theorems we proved above. Algorithmically, we simply sample $q$ rows and columns of our matrix and output the corresponding norm of the sub-matrix as our estimate. 


\ainesh{Instead of using the main theorem, we should equation 36 to bound the expectation, and use the main theorem to bound the variance}



==> scrap.tex <==
%!TEX root = ../main.tex


\begin{lemma}(Spectral Approximation via Column Sampling.) Sampling $t = \frac{c'\sqrt{k/\alpha}}{\epsilon^2}\log\left(\frac{2n}{\delta}\right)$ columns of $\AA$ uniformly and scaling each column by $\sqrt{n/t}$ results in a matrix $\CC$ such that
with probability $1-\delta$, 
\[
(1-\epsilon)\AA\AA^T  - \frac{\epsilon}{k}\| \AA\|^2_F \II \preceq \CC \CC^T \preceq (1+\epsilon)\AA\AA^T +  \frac{\epsilon}{k}\| \AA\|^2_F\II
\]
\end{lemma}
%=  O\left(\frac{ m}{b\epsilon^2}\log(\frac{m}{\delta})\right)
\begin{proof}
Consider the random variable $\Y = \CC\CC^T - \AA\AA^T = \sum_{j \in [t]} \left(\CC_{*,j} \CC_{*,j}^T -\frac{1}{t}\AA\AA^T\right) = \sum_{j\in [t]} \X_j$. Recall, $\CC_j = \sqrt{n/t}\AA_j$ and thus $\X_j = \frac{1}{t}(n\AA_{j}\AA^T_{j} - \AA\AA^T )$ with probability $1/n$. We observe that $\expec{}{\X_j} = \expec{}{\CC_{*,j} \CC_{*,j}^T -\frac{1}{t}\AA\AA^T}= \left(\sum^n_{j =1}\AA_{*,j}\AA_{*,j}^T \right) - \AA \AA^T= 0$, and therefore, $\expec{}{\Y} =0$. Next, we bound the operator norm of $\Y$ using the Matrix Bernstein inequality. 
Let $\|\AA_{j^*} \|^2_2 = \max_{j \in [n]} \|\AA_j\|^2_2$. 
We begin by showing an upper bound on the operator norm of $\X_j$:
\begin{equation}
\label{eqn:spec_x_j}
    \begin{split}
        \| \X_j \|_2 
        \leq \frac{n}{t} \|\AA_{j}\AA^T_{j} \|_2 + \frac{1}{t} \| \AA\AA^T \|_2
         \leq  \frac{n}{t}\|\AA_{j^*}\|^2_2 + \frac{1}{t}\| \AA \|^2_2
    \end{split}
\end{equation}
where we use that for a rank-$1$ matrix, $\|u u^T\|_2 = \|u\|^2_2$ and $\| \AA \|_2 = \max_{\|x\|_2=1} | x^T \AA x | \leq (\sum_{i\in[n]} x_i)^2 \leq n$.
Next, we bound $\var{\Y}\leq \expecf{}{\Y^2}$.

\begin{equation}
\label{eqn:variance_bound}
    \begin{split}
        \expecf{}{\Y^2}  =  t\expecf{}{\left(\CC_{*,j} \CC_{*,j}^T -\frac{1}{t}\AA\AA^T\right)^2} 
        & = t\expecf{}{ \left(\CC_{*,j} \CC_{*,j}^T\right)^2 +\frac{1}{t^2}\left(\AA\AA^T\right)^2 - \frac{2}{t}\CC_{*,j} \CC_{*,j}^T \AA\AA^T } \\
        & = t \left(\sum_{j \in [n]} \frac{q_j}{t^2q_j^2} (\AA_{j}\AA^T_{j})^2 + \frac{1}{t^2}(\AA\AA^T)^2 - \sum_{j \in [n]} \frac{2q_j}{q_j t^2} \AA_j \AA_j^T \AA \AA^T \right) \\
        & = \frac{1}{t}\left( \sum_{j \in [n]} \frac{(\AA_{j}\AA^T_{j})^2}{q_j} + (\AA\AA^T)^2 - \sum_{j \in [n]} 2 \AA_{j}\AA^T_{j} \AA\AA^T \right) \\
        & = \frac{1}{t}\left( \sum_{j \in [n]} \frac{(\AA_{j}\AA^T_{j})^2}{q_j} - (\AA\AA^T)^2 \right) \\
        & \preceq \frac{n}{t}\left( \sum_{j \in [n]} (\AA_{j}\AA^T_{j})^2 \right) \\
        & \preceq \frac{n}{t}\left( \sum_{j \in [n]} \| \AA_{j^*}\|^2_2 (\AA_{j}\AA^T_{j}) \right) \\
        & \preceq \frac{n\|\AA_{j^*}\|^2_2}{t} \AA \AA^T \\
    \end{split}
\end{equation}
where we use linearity of expectation, $(\AA\AA^T)^2 \succeq 0$.
We first consider the case where $\|\AA_{j^*}\|^2_2 \leq \|\AA\|_2$. We can then bound $\| \X_j \|_2 \leq \frac{2n}{t}\| \AA\|_2$ in \eqref{eqn:spec_x_j}, where we use $\|\AA \|_2 \leq n$. Further,   $ \Big\| \expecf{}{\Y^2} \Big\|_2 \leq \frac{cn\|\AA \|^3_2 }{t}$ in \eqref{eqn:variance_bound}.
Applying the Matrix Bernstein inequality, 



\begin{equation*}
    \begin{split}
        \prob{}{\| \Y \|_2 \geq \Big\|\epsilon \AA\AA^T  +  \frac{\eps}{k} n^2 \II \Big\|_2 } & \leq 2n \exp{\left(- \frac{\big\|\epsilon \AA\AA^T  +  \frac{\epsilon n^2}{k}\II \big\|^2_2}{  \frac{n \|\AA_{j^*}\|_2^2 \|\AA \|^2_2 }{t}  +  \frac{(\frac{n}{t}\|\AA_{j^*}\|^2_2 + \frac{1}{t}\| \AA \|^2_2) \left(\big\|\epsilon \AA\AA^T  +  \frac{\epsilon n^2}{k} \II \big\|_2 \right)}{3t} }\right)} \\
        & = 2n \exp{\left(-\frac{\epsilon^2 }{k^2 }\left(  \frac{\big\|k \AA\AA^T  + \|\AA\|^2_F \II \big\|^2_2 }{ \frac{cn \|\AA \|^3_2 }{t}  +  \frac{2\epsilon n \|\AA\|_2 \left(\|k \AA\AA^T  + \|\AA\|^2_F \II \|_2 \right)}{3kt}}\right) \right)} \\
        & = 2n \exp{\left(-\frac{\epsilon^2t }{c'k^2n \|\AA \|_2 }\left(  \frac{\big\|k \AA\AA^T  + \|\AA\|^2_F \II \big\|^2_2 }{ \frac{ k\|\AA\AA^T \|_2 + \epsilon \|k \AA\AA^T  + \|\AA\|^2_F \II \|_2  }{k}}\right) \right)} \\
        & \leq 2n \exp{\left(-\frac{\epsilon^2t }{c'kn \|\AA \|_2 }\left(  \frac{\big\|k \AA\AA^T  + \|\AA\|^2_F \II \big\|^2_2 }{(1+\epsilon) \|k \AA\AA^T  + \|\AA\|^2_F \II \|_2  }\right) \right)} \\
        %& = 2n \exp{\left(- \frac{3 \epsilon^2 \| \AA \|^2_F t}{cn \|\AA\|_2 (1+\epsilon)} \right)} \\
        & \leq 2n \exp{\left(- \frac{ \epsilon^2 t \left( \big\|k \AA\AA^T  + \|\AA\|^2_F \II \big\|_2 \right) }{c'nk \|\AA\|_2 } \right)} \\
        & \leq 2n \exp{\left(- \frac{ \epsilon^2 \sqrt{k}t \| \AA \|_2 \|\AA\|_F }{c'nk \|\AA\|_2 } \right)} \hspace{0.5in} \textrm{ [A.M - G.M inequality]}\\
        %& \leq 2n \exp{\left(- \frac{3 \epsilon^2 t \sqrt{n}}{cn } \right)} \\
        & \leq 2n \exp{\left(- \frac{\epsilon^2 \sqrt{\alpha} t}{c'\sqrt{ k} } \right)} \\
        %& \leq 2n \exp{\left(- \frac{\epsilon^2 \| \AA \|_F t}{cn} \right)} \\
        %& \leq 2n \exp{\left(- \frac{\epsilon^2  t}{c\sqrt{n}} \right)} \\
        %&\leq \delta
    \end{split}
\end{equation*}
Here, we use $\|k \AA\AA^T  + \|\AA\|^2_F \II \|_2 = k\|\AA \|^2_2 + \|\AA\|^2_F \geq 2 \sqrt{k} \|\AA \|_2\|\AA\|_F$, by the AM-GM inequality. Next, we use  $\|\AA\|_F\geq \sqrt{\alpha} n$ by assumption. In order to bound the error probability by $\delta$ we set $t = \frac{c'\sqrt{k/\alpha}}{\epsilon^2}\log\left(\frac{2n}{\delta}\right)$. Therefore, with probability $1-\delta/2$, 
\begin{equation}
(1-\epsilon)\AA\AA^T  - \frac{\epsilon}{k}\| \AA\|^2_F \II \preceq \CC \CC^T \preceq (1+\epsilon)\AA\AA^T +  \frac{\epsilon}{k}\| \AA\|^2_F\II
\end{equation}

Next, consider the case where $\|\AA\|_2 \leq \|\AA_{j^*}\|^2_2$. Then, $\|\X_j\|_2 \leq \frac{2n}{t} \|\AA_{j^*}\|^2_2$ and $\| \expec{}{\Y^2}\|_2 \leq \frac{n}{t} \|\AA_{j^*}\|^2_2\|\AA\|^2_2$. Applying Matrix Bernstein again, we have 
\begin{equation*}
    \begin{split}
        \prob{}{\| \Y \|_2 \geq \Big\|\epsilon \AA\AA^T  +  \frac{\epsilon}{k}\| \AA \|^2_F\II \Big\|_2 } & \leq 2n \exp{\left(-\frac{\epsilon^2 }{k^2 }\left(  \frac{\big\|k \AA\AA^T  + \|\AA\|^2_F \II \big\|^2_2 }{ \frac{cn \|\AA_{j^*}\|^2_2\|\AA\|^2_2 }{t}  +  \frac{2\epsilon n \|\AA_{j^*}\|^2_2 \left(\|k \AA\AA^T  + \|\AA\|^2_F \II \|_2 \right)}{3kt}}\right) \right)} \\
        & \leq 2n \exp{\left(- \frac{ \epsilon^2 t \left( \big\|k \AA\AA^T  + \|\AA\|^2_F \II \big\|_2 \right) }{c'nk \|\AA_{j^*}\|^2_2 } \right)} \\
        & \leq 2n \exp{\left(- \frac{ \epsilon^2 \alpha t n^2 }{c'k n^2 } \right)} \\
    \end{split}
\end{equation*}
Setting $t = k/\alpha\epsilon^2\log(n/\delta)$ and union bounding over the failure probability in both cases to conclude that with probability $1-\delta$
\[
(1-\epsilon)\AA\AA^T  - \frac{\epsilon}{k}\| \AA\|^2_F \II \preceq \CC \CC^T \preceq (1+\epsilon)\AA\AA^T +  \frac{\epsilon}{k}\| \AA\|^2_F\II
\]
\end{proof}




\begin{comment}
\section{Multiple Negative Eigenvalues in the Sensing model}
Let $A \in \R^{n \times n}$ be a symmetric matrix with eigenvectors $v_1,v_2,\dots,v_m$, for $m \leq n$, and eigenvalues $\lambda_1 \leq \lambda_2 \leq \dots \leq \lambda_k < 0 \leq \lambda_{k+1} \leq \dots \leq \lambda_m$. Note that $\|A\|_F^2 = \sum_{i=1}^m \lambda_i^2$. Now let $\eps = \frac{ \sum_{i=1}^k \lambda_i^2}{\|A\|_F^2} \leq 1$, which is a measure of the fraction of $A$ that is negative. We consider the sensing model, where the algorithm fixes sensing matrices $X_1,\dots,X_\ell \in \R^{n \times n}$ and observes $\rho_i \langle \text{vec}(X_i), \text{vec}(A) \rangle = \text{Tr}(X_i^T A)$. Thus the observation $\rho_i$ is a linear function of the enties of $A$. 

\begin{theorem}
    There is an algorithm in the sensing model which uses $\ell = O(1/\eps^2)$ observations and tests whether $A$ is PSD or if $\frac{ \sum_{i=1}^k \lambda_i^2}{\|A\|_F^2} \geq \eps$.
\end{theorem}
\begin{proof}
We first describe our sketching matrices $X_1,\dots,X_\ell$. First, we generate Gaussian vectors $g_1,g_2,\dots,g_r \in \mathcal{N}(0,\mathbb{I}_n)$, for $r = \Theta(1/\eps^2)$. First note that the length of the projection of $g_i$ onto $v_j$ can be written as $\langle v_j, g_i \rangle = h_{i,j} \sim \mathcal{N}(0,1)$ since $v_j$ is a unit vector.
Thus if $h_i \in \R^n$ is the vector such that $(h_{i})_j = h_{i,j}$, we can write $V^T g_i = h_i$, where $V \in \R^{n \times m}$ is the matrix with $j$-th column equal to $v_j$. Since $V^T$ now has orthogonal rows, it follows that $h_{i,1},h_{i,2},\dots,h_{i,m}$ are i.i.d. standard Gaussian variables. 

By the prior paragraph, we can write $g_i$ as the projection of its components onto the eigenspace of $A$ $g_i = \sum_{j=1}^m v_j v_j^T h_{i,j} + \beta_i$, where $\beta_i \in \R^n$ is in the null space of $A$. Thus
\[  g_i^T A g_i =     \sum_{j=1}^m \lambda_j h_{i,j}^2   \] 
Moreover, $\ex{ (g_i^T A g_i)^2 } = \sum_{j} \lambda_j^2 $, which holds since the $h_{i,j}$'s are independent and mean $0$ variance $1$.


We create a sketching matrix $X_i$ for each quadratic form, so that $\langle X_i, A\rangle = g_i^T A g_i$.

\end{proof}
\section{Spread Eigenvalue PSD testing}

\section{Cut Norm}
Using Veryshin expectation upper bound

Cut norm is $\max_{x,y \in \{0,1\}^n} |y^\top A x|$.x
\begin{theorem}
	There is an algorithm that gives an $O(1)$ relative error approximation of the cut norm by only looking at $O(n^4/\|A\|_C^2)$ entries of $A$. 
\end{theorem}

\section{Schatten $p$-norm}
\section{Operator norm}

The operator norm of $A \in \R^{n \times m}$ is given by $\|A\|_2 = \max_{x \in \R^m: \|x\|_2 = 1} \|Ax\|_2$. Note that $\|A\|_2$ can also be written by
\[	\|A\|_2 = \max_{y \in \R^m, x \in \R^n, \|x\|_2 = \|y\|_2 = 1} |y^\top A x|	\]
\begin{proof}
	
We first prove $\|A\|_2 \leq$ the RHS. To see this, let $x$ be such that $\|Ax\|_2 = \|A\|_2$. Then if we set $y = Ax/\|Ax\|_2$, then we have $y^\top Ax = \|Ax\|_2$, which completes the proof of this direction. Now to see that $\|A\|_2 \geq$ the RHS, fix $x,y$ that maximizes $y^\top A x$. For any $x$, the $y$ that maximizes $y^\top A x$ is $y=Ax/\|Ax\|_2$, thus $y^\top A x = \|Ax\|_2 \leq \|A\|_2$ as needed.
\end{proof}

Fix $x,y$ such that $yAx = \|A\|_2 $. We now computed the expectation of $y_T A x_S$, where $|T| = |S| = k$ are independent, uniform samples of $[n]$. Let $\delta_i$ indicate we sample the $i$-th column, and let $\theta_i$ indicate we sample the $i$-th row. with $\ex{\delta_i} =p, \ex{\theta_i} = q$, such that $pq = \frac{k^2}{n^2}$, where $k = \Theta(1/\eps)$. The following is clear. 
\begin{proposition}
		We have \[ \bex{\sum_{i ,j} y_i A_{i,j} x_i\theta_i \delta_j } = pq\left(yAx\right) = \frac{k^2}{n^2} \|A\|_2	 = \frac{\eps k^2}{n}\]
\end{proposition}
Let  $c_{i,j} = y_i A_{i,j} y_j$, and define the row and column contributions as $\RR_i = \sum_{j \in [n]} c_{i,j}$ 
$\CC_i = \sum_{j \in [n]} c_{j,i}$.
\begin{lemma}\label{lem:spectralvar}
	Assuming $k = \Omega(1/\eps)$, we have 	\[\mathbf{Var}\left[\sum_{i,j} y_i A_{i,j} y_j \delta_i \delta_j	\right] \leq  pq + 2\sum_i \left( p q^2  \RR_i^2 +  p^2 q \CC_i^2  \right) \]
\end{lemma}
\begin{proof}
. Then we have
	\begin{equation} 
\begin{split}
&\mathbf{Var}\left[\sum_{i,j} y_i A_{i,j} y_j \delta_i \delta_j	\right] \leq  pq\sum_{i , j} c_{i,j}^2  + p q^2\sum_{i } \sum_{j  \neq v} c_{i,j} c_{i,v} +  p^2 q \sum_j \sum_{i \neq u} c_{i,j} c_{u,j}  \\
%+& \frac{k^2}{n^2} \sum_{i \neq j}c_{i,i}c_{j,i} + \frac{k^3}{n^3}\sum_{i\neq j \neq u} c_{i,j} c_{u,j}  + \frac{k^3}{n^3}\sum_{j\neq i \neq u} c_{i,j} c_{i,u}  + \frac{k^3}{n^3}\sum_{i\neq j \neq u} c_{i,j} c_{j,u}+ \frac{k^3}{n^3}\sum_{j\neq i \neq u} c_{i,j} c_{u,i} \\ 
&  + p^2 q^2\sum_{ i \neq u, u \neq v} c_{i,j} c_{u,v}  - \left( pq\sum_{i, j} y_i A_{i,j} y_j \right)^2 \\
\end{split}
\end{equation}
Similar to proposition \ref{prop:var}, we can cancel the $p^2 q^2\sum_{ i \neq u, u \neq v} c_{i,j} c_{u,v}$ term with the expectation squared, and the remaining terms from the latter can be upper bounded by bounding the first three terms. First, note $\sum_{i , j} c_{i,j}^2  \leq \sum_{i , j} y_i^2 y_j^2 \leq 1$, so $ pq\sum_{i , j} c_{i,j}^2 \leq pq$. Next  $\sum_{i } \sum_{j  \neq v} c_{i,j} c_{i,v} \leq \RR_i^2 + \sum_{i=1}^n y_i^2 \leq \RR_i^2 + 1$, where $\RR_i = \sum_{j \in [n]} c_{i,j}$. Similarly $\sum_j \sum_{i \neq u} c_{i,j} c_{u,j} \leq \CC_i^2 + 1$, thus 
	\[\mathbf{Var}\left[\sum_{i,j} y_i A_{i,j} y_j \delta_i \delta_j	\right] \leq  pq + 2\sum_i \left( p q^2  \RR_i^2  +  p^2 q \CC_i^2  \right) \]

	where  the extra factor of $2$ comes from absorbing possibly positive terms in minus the expectation squared, as well as the $+1$ term.
\end{proof}

We now consider two cases. First suppose that for every $S,T \subseteq [n]$ with $|S|,|T| \leq - \eps n/10$, we have $y_{-S} A x_{-T} \geq \eps n/ 2$. Call this case $1$.

\begin{lemma}
	Suppose we are in case $1$. Then there is an algorithm that samples $\ell$ $k \times k$ submatrix $Z_1,\dots,Z_{\ell}$ of $A$, where $\ell = O(1)$ and $k = \Theta(1/\eps)$, such that $\frac{1}{\ell}\sum_{i=1}^\ell\|Z_i\|_2 \geq \frac{k}{n} \|A\|_2$, or  $$\frac{200n}{k\ell}\sum_{i=1}^\ell\|Z_i\|_2 \geq \|A\|_2$$
\end{lemma}
\begin{proof}		
	We first claim that we can modify $x,y$ so that $y A x \geq \eps n/2$, and such that $\sum_i \RR_i^2 + \CC_i^2 \leq O(\eps n)$
	Now by the assumption on the case, we can first remove a set
	Sets $S_0 = \{i \in [n] \; | \; |y_i| \geq \frac{10}{\sqrt{ \eps n}} \}$ and $T_0 = \{i \in [n] \; | \; |x_i| \geq \frac{10}{\sqrt{ \eps n}}\}$, which each have size at most $\eps n / 100$. Moreover, we will still have $y_{-S_0} A x_{-T_0} \geq \eps n /2$, and $\|x\|_\infty, \|y\|_\infty \leq \frac{10}{\sqrt{ \eps n}}$.	Afterwards, note that we can assume $\RR_i^2 > 0$ (and $\CC_i > 0$), since otherwise we could set $y_i$ (or $x_i$) equal to $0$, and only increase $yAx$. Moreover, note that $\sum_i| \RR_i| =\sum_i \RR_i\leq \eps n$ and $\sum_i \CC_i \leq \eps n$. 
	
	Now define
	 $S = \{i \in [n] \; | \; |\RR_i| \geq 10 \} \cup S_0$, which has size at most $|S| \leq \eps n / 10$, and remove the coordinates in $S$ from $y$ (set them equal to zero). Afterwards, the result is that $\max_i |\RR_i| \leq 10$. Next, we can remove $T = \{i \in [n] \; | \; |\CC_i| \geq 10 \} \cup T_0$ from $x$, and have $\max_i |\CC_i| \leq 10$. Now the second step can increase the value of a given $|\RR_i|$, but only by at most $(\eps n/10)|x|_\infty |y|_\infty \leq  10$. It follows that after these modifications, we have $\max_i |\RR_i| \leq 20$ and $\max_i |\CC_i| \leq 10$, and moreover $y_{-S} A x_{-T} \geq \eps n/2$. Define these to be our new vectors. Putting together the $\ell_\infty$ and $\ell_1$ bounds on the $\RR_i$ and $\CC_i$, we have $\sum_i \RR_i^2 + \CC_i^2 \leq \eps 30 \eps n$.  
	 
	 Now by Lemma \ref{lem:spectralvar}, if we set $p=q=\frac{k}{n}$, it follows that $\bvar{ \sum_{i,j} (y_{-S})_i A (x_{-T})_j \theta_i \delta_j } \leq \frac{k^2}{n^2} + \frac{k^3}{n^3} (30 \eps n)$. Since $k=\Theta(1/\eps)$, the result is that the variance is $O(k^2/n^2)$ and the expectation is $\frac{k^2}{n^2} \|A\|_2	 =O(k/n)$, so the average is at least $\frac{k^2}{n^2} \|A\|_2	/2$ with probability $9/10$. By Markov's, the $\ell_2$ of the sampled coordinates in $x,y$ in each repetition was at most $100\frac{k}{n}$, thus we have that $\frac{1}{\ell}\sum_{i=1}^\ell\|Z_i\|_2 \geq \frac{k}{200n}\|A\|_2$, or 
	 $$\frac{200n}{k\ell}\sum_{i=1}^\ell\|Z_i\|_2 \geq \|A\|_2$$
\end{proof}

\begin{lemma}
	Suppose we are not in case $1$. Then there is an algorithm that samples $\ell$ submatrix $Z_1,\dots,Z_{\ell}$ of $A$, each of which has total size $O(\log^2(1/\eps)/\eps^2)$ and $\ell = O(\log(1/\eps))$, such that \[\max_i \|Z_i\|_2 \geq \frac{k}{600 \log(1/\eps) n} \|A\|_2\]
	 \end{lemma}
\begin{proof}
	Suppose we are not in case $1$. First note that for any sets $S,T$ with size at most $\eps n/10$, the contribution of $y_S A x_T$ is at most $\eps n/10$, thus if we are not in case $2$, then wlog there is a set $S$ with $|S| \leq \eps n/10$ such that $y_S A x \geq \eps n /6$. First note that we can assume that $S \subseteq T_a = \{ i \in [n] : \; : \frac{2^a}{n} \leq |y_i|^2 \leq \frac{2^{a+1}}{n} \}$ for some $1 \leq a \leq \log(1/\eps)$, at the cost of  $y_S A x \geq \eps n /24 \log(1/\eps)$. We can now sample a submatrix of $y_S A x$ of size $k^2$, which has expected value at least $\frac{k^2}{n^2} \|A\|_2/(24 \log(1/\eps))$.  
	
	
We now consider the variance of this sampling. As before, we can assume $\RR_i > 0$ for all $i$. Now first observe  $\sum_i \CC_i^2 \leq \sum_{i } x_i^2 \left(\sum_{j \in S}A_{j,i}y_j	  \right)^2 \leq\sum_{i } x_i^2 \|y_{S}\|_1^2 \leq |S|$. Moreover, we have $\RR_i \leq  y_i |x|_1 \leq \|y\|_\infty \sqrt{n}$, and $\sum_i |\RR_i| \leq \eps n$, as well as $\|y\|_\infty^2 \leq \frac{2^a}{n}$. So we have $\max_i |\RR_i|^2 \leq 2^a$, thus $\sum_i \RR_i^2 \leq   (\eps n/ \sqrt{2^a})(2^a) \leq \eps n \sqrt{2^a}$.  
	
	We can now sample with $p = \frac{1}{|S|}$ and $q = \frac{|S| k^2}{n^2}$. so that $pq = \frac{k^2}{n^2}$. Firstly, note that the $2\sum_i p^2 q\CC_i^2$ term in the variance is at most $\frac{k^2}{|S| n^2} |S| = \frac{k^2}{n^2}$, and the term $2 \sum_i pq^2\RR_i^2 \leq2 \frac{k^4 |S|}{n^4} ( \eps n 2^{a/2}) \leq 2\frac{ \eps k^4 |S| 2^{a/2}}{n^3} \leq 2\frac{\eps k^4 }{2^{a/2}n^2}$, where the last inequality holds because $|S| \leq |T_a| \leq n/2^a$.   Now first note that we can assume that $2^{a/2} \geq 1/(100\eps)$. If we could not choose such an $a$, then we would have $y_SAx \leq - \eps n / 12$, but since $S$ has size at most $\eps n / 100$, we have $\|y_s\|_2 \leq 1/100$, and we could scale $y$ by a factor of $100$ entrywise and obtain $yAx \geq 10\eps n = 10 \|A\|_2$ where $x,y$ are still at most unit vectors, which is impossible. Thus $2 \sum_i pq^2\RR_i^2 \leq \frac{2 \eps^2 k^4}{n^2 } = \frac{2 \|A\|_2^2 k^2}{n^4}$. 
	
Altogether, the variance is at most $2 \frac{k^2}{n^2} + \frac{2 \|A\|_2^2 k^2}{n^4} \leq \frac{4 \|A\|_2^2 k^2}{n^4}$. Now note that the expectation of the sampling is at least $\frac{k^2}{n^2} \|A\|_2 /(24 \log(1/\eps))$, and since $k \geq \log(1/\eps)/\eps$, it follows that, with probability at least $9/10$, we have that a single sample satisfies $\sum_{i,j}c_{i,j} \theta_i \delta_j \geq  \frac{k^2}{n^2} \|A\|_2 /(30 \log(1/\eps))$. Moreover, note that the expected $\ell_2^2$ of the coordinates of $y$ is $p$, and for $x$ it is $q$. With probability $9/10$, we have both that the $\sum_i y_i^2 \theta_i \leq 20p$ and $\sum_i x_i^2 \delta_i \leq 20q$. Thus we can scale each coordinate $y_i$ by $1/\sqrt{20 p}$ and each $x_i$ by $1/\sqrt{20 q}$, which scales the whole quadratic form by $\frac{1}{10 \sqrt{pq}} = \frac{n}{20k}$. Thus we have $\sum_{i,j}c_{i,j} \theta_i \delta_j \geq  \frac{k}{n} \|A\|_2 /(600 \log(1/\eps))$ after this scaling, with probability $4/5$. It follows that with constant probability, the spectral norm of this sampled submatrix is at least  $\frac{k}{n} \|A\|_2 /(600 \log(1/\eps))$ with constant probability, and we must repeat once for each of the $\log(1/\eps)$ guesses of the sampling probabilities $p$. 
	
	
%	 Thus the variance is at most $\log^2(1/\eps) \frac{k^2}{n^2}$, and the expectation is $\frac{ k}{n} \|A\|_2/24 $. So we can repeat $\log^2(1/\eps)$, and get a sample with value at least $\frac{ k}{n} \|A\|_2/24 $ with large constant probability. We can then repeat this for $\log(1/\eps)$ guesses of $|S|$ to get the desired result. By Markov's, the $\ell_2$ of $x,y,$ on the subsampled parts blows up by at most $\log(1/\eps)$ on the right level of sampling, so it follows that $\|Z_i\|_2 \geq (\frac{k^2}{n^2} \|A\|_2/\log(1/\eps) ) \frac{n}{\log^2 (1/\eps)} = \frac{k}{n \log^3(1/\eps)} \|A\|_2$ (actually because of the way the sampling ratio vs level sets work, the $\ell_2$ of a sample concentrates!). 
\end{proof}

Putting the two results together, we obtain:

\begin{theorem}
There is an algorithm that samples $\ell = O(\log(1/\eps))$ submatrices $Z_1,\dots,Z_{\ell}$ of $A$, each of which has at most $O(\log^2(1/\eps)/\eps^2)$ entries,  such that \[\max_i \|Z_i\|_2 \geq \frac{k}{600 \log(1/\eps) n} \|A\|_2\]
\end{theorem}


\begin{lemma}
	We have 
	\[	\bex{\|A_{S \times T}\|_2} \leq O\left(\frac{k}{n} \|A\|_2 + \sqrt{k} \right)	\]
\end{lemma}

It follows that 
 $$\frac{200n}{k\ell}\sum_{i=1}^\ell\|Z_i\|_2 \leq O\left(\|A\|_2(1 + \frac{1}{\eps\sqrt{k} })\right)$$

So we obtain an estimate $\Psi$ with 

\[\|A\|_2	\leq	\Psi \leq C_1 \|A\|_2(1 + \frac{1}{\eps\sqrt{k} })\]


\end{comment}

